The Endokernel: Fast, Secure, and Programmable Subprocess Virtualization

Commodity applications contain more and more combinations of interacting components (user, application, library, and system) and exhibit increasingly diverse tradeoffs between isolation, performance, and programmability. We argue that the challenge of future runtime isolation is best met by embracing the multi-principle nature of applications, rethinking process architecture for fast and extensible intra-process isolation. We present, the Endokernel, a new process model and security architecture that nests an extensible monitor into the standard process for building efficient least-authority abstractions. The Endokernel introduces a new virtual machine abstraction for representing subprocess authority, which is enforced by an efficient self-isolating monitor that maps the abstraction to system level objects (processes, threads, files, and signals). We show how the Endokernel can be used to develop specialized separation abstractions using an exokernel-like organization to provide virtual privilege rings, which we use to reorganize and secure NGINX. Our prototype, includes a new syscall monitor, the nexpoline, and explores the tradeoffs of implementing it with diverse mechanisms, including Intel Control Enhancement Technology. Overall, we believe sub-process isolation is a must and that the Endokernel exposes an essential set of abstractions for realizing this in a simple and feasible way.

==> acks.tex <==
%-------------------------------------------------------------------------------
\section*{Acknowledgments}
%-------------------------------------------------------------------------------

The USENIX latex style is old and very tired, which is why
there's no \textbackslash{}acks command for you to use when
acknowledging. Sorry.



==> alt-intro.tex <==
\section{Introduction}

  % --------------------
  Traditionally, modularity is provided using virtualization, where the
  underlying CPU and physical memory are virtualized as a virtual machine.
  %
  Hardware and the OS combine to provide the illusion that a thread of execution
  has the full machine.
  %
  The basic abstraction for doing this is the process, where multiple threads of
  execution share memory and OS virtual objects.
  %
  The problem is that processes are large and fail to apply least-authority
  design.
  %
  This means that malicious components or any native code compromise will allow
  an attacker access to the full authority of the process.

  % --------------------
  Privilege separation is an approach that decomposes
  applications into multiple modules to gain the isolation
  benefits of modularity.
  %
  The basic idea is to take things that were once in a
  single virtual machine and split it into multiple and
  present fine-grained isolation than the application.
  %
  Unfortunately, process level isolation, as used by bla bla
  bla, is very slow, thus significantly restricting it's
  applicability in practice.
  %
  Instead, nested isolation has been chosen.
  %
  However, when nesting, the system naturally multiplexes
  privileges within the standard process/thread abstraction,
  which is breaks assumptions by the OS.
  %
  These assumptions then lead to many security
  vulnerabilities. 
  %
  What we need is a proper and complete consideration of
  what resources must be virtualized across OS abstractions
  and address several low-level considerations neglected
  because these runtimes neglected standard OS abstractions
  (concurrency, threading, etc). 

  % --------------------
  Isolation depends on identifying and virtualizing
  (interposing/monitoring/etc) all resources that allow
  information to flow-to or be accessed-by unintended
  recipients.
  %
  In a computing system we consider processes and users as
  principles, thus, current granularity to distinguish
  principles is greatly hindered by the process abstraction
  and modern software development methods.
  %
  Our goal is to allow the methods to remain while
  automatically or with minimal effort adding in isolation.
  %
  To do so we nest an isolation manager, \ie separation
  kernel, into the process space.
  %
  The Nested
  Visor/endovisor/nestedvisor/isovisor/intravisor/\ldots
  architecture does so by virtualizing cpu and memory state
  that otherwise allows the visor to be circumvented.
  %
  Next we use that to do isolation in the process. 


==> archive.tex <==

  % --------------------
  %\paroutline{Context}{Single-Address Space Privilege Sep}
  %
  Privilege separation decomposes an application into separate compartments so
  that each has a least-privilege~\cite{Miller:Robust:2006,
  Saltzer:Protection:1975} view of memory; and has been used to ensure
  resiliency to Trojan~\cite{Karger:Limiting:1987} and control-flow
  hijack~\cite{Szekeres:SoK:2013} attacks.
  % --------------------
  Beyond the many benefits of modularity~\cite{encapsulation}, privilege
  separation can even weaken, if not altogether prevent, attacks like
  HeartBleed~\cite{Durumeric:Matter:2014}, SolarWinds~\cite{Solarwinds}, and the
  recent Sudo exploit~\cite{baronsamedit2021} (a Sudo exploit defense is
  presented in \S~\ref{sec:usecase}).
  %
  Early approaches manually decomposed and used address-space
  isolation~\cite{Vasilakis:Automated:2018, Provos:Preventing:2003,
  Litton:Lightweight:2016, Bittau:Wedge:2008, Hsu:Enforcing:2016}, however,
  effective separation requires object-level isolation, which is too complex to
  specify policies for and slows too much.
  %
  In response, a 3rd generation~\cite{Hsu:Enforcing:2016} of solutions combine
  novel hardware mechanisms with language based techniques to \emph{nest} the
  \monitor inside the address space~\cite{Dautenhahn:Nested:2015,
    Vahldiek-Oberwagner:ERIM:2019, Hedayati:Hodor:2019, Park:libmpk:2019,
  Liu:Thwarting:2015, Koning:No:2017, Chen:Shreds:2016, Hsu:Enforcing:2016}.

  % --------------------
  %\paroutline{Gap}{Missing Implicit Flows}
  %
  %but stay within the threat model~\cite{Connor:PKU:2020}.
  %
  \iftrue % ndd: couldn't decide, so save these for analysis later
  %
  Unfortunately, these efforts neglect several implicit information flows that
  bypass monitoring but stay within their threat models~\cite{Connor:PKU:2020}.
  %
  \else
  %
    ---information can still implicitly flow into or out of a protected
    \segment.
    %
    ---the OS allows memory to be mapped as pseudo files, allows protection
    changes to memory, or even signals can create exploitable control
    flows~\cite{Connor:PKU:2020} (depicted in Figure~\ref{fig:problem}).
    %
    %
  %
  Unfortunately, prior work only monitors memory access, which is only one way
  to access information in a process, \ie data is accessible through system
  objects and CPU registers, which can be used by attackers to bypass privilege
  separation~\cite{Connor:PKU:2020}.
  %
  %memory access is only one way to access a process's information---
  %
  %Unfortunately, memory protection only prevents one way of accessing
  %information, it neglects data flows through both system
  %objects~\cite{Connor:PKU:2020} and CPU registers, which can be used by
  %attackers to bypass \nemo policies.
  %
  \fi
  %
  These flows result from 1) the lack of a \subdomain abstraction in the kernel,
  leading to leaky system objects, and 2) missing abstractions in the \nemo
  mechanisms, leading to low-level exploits.
  %
  First, system objects allow bypass through signals, \syscalls, and forked
  address-spaces.
  %
  For example, suppose \Code{s} points at an isolated session key, then the
  following pseudo code would bypass any memory protection:
  % --------------------
  \begin{lstlisting}[language=C,style=customc]
  open("/proc/self/mem","r").seek(s).read(0x10) \end{lstlisting}
  %
  Signals expose protection information in virtual CPU state (\eg
  \Code{pt\_regs}) and can be used to coerce control and data flow.
  %
  Second, prior work neglects full implementation and analysis of multi-threaded
  concurrency and multi-domain separation, which means several access paths are
  left undefended: without implementing concurrency, \monitor state can be
  corrupted or security checks bypassed and in multi-domain the context switch
  exposes attacker controllable registers.
  %
  Table~\ref{tbl:barf} and Figure~\ref{fig:problem} summarize key differences
  and limitations of prior work.

  % --------------------
  \begin{figure}[!b]
      %
      \begin{center} \includegraphics[width=.9\textwidth]{figs/problem}
      \end{center}
      %
      \caption{\label{fig:problem}
        %
        Problem: intra-process is bypassable because domain is opaque to OS,
        sandbox limits functionality, and inter-process is slow and costly to
        apply. Red indicates limitations.
        %
      } \vspace{-3mm}
  %
  \end{figure}




\iffalse

  \review{THIS paragraph hastily spliced and written from several prior things.
    It maybe makes sense in some paragraphs. Maybe not. It tries to get a vague
    organization of how to describe things, then gave up and just pulled in
    other stuff. There is a need to intro the sys flow policies with context,
  likely introducing some of our analysis? Not sure.}

  What is the basic design/org and management of the \visor architecture?
  Policies? Properties? etc.

  This details the mechanism independent arch, ie could be implemented with
  sfi/cfi, address space iso, ept, mpk, etc. So the overarching theme is to
  distinguish elements that are helpful in moving these architectures forward:
  what do others miss? That is the key here. The most novel is the syscall
  policies and basic requirement specification for what to virtualize: what's
  the set of necessary primitives\ndd{how is this diff from priv model?}

  \ndd{I'm not sure we can actually argue for an arch independent abstraction.
   The problem is instruction capapbilities. Without these we basically just
 have a micro kernel and aren't too interesting.}

  %
  \iffalse
  % --------------------
  In 2003 Niels Provos pointed out that, ``We take for
  granted that applications will always contain exploitable
  bugs that may lead to unauthorized
  access''~\cite{Provos:Improving:2003}, and although
  certainly nothing has gotten better, arguably it has
  gotten worse with today's large application ecosystems.
  %
  \fi

  % --------------------
  %\paroutline{Trend}{Intra-process iso is growing and
  %necessary}
  %
  A growing body of production systems and research rely on
  intra-process isolation to provide lightweight sandboxing
  of untrusted code.
  %
  Google's NaCL~\cite{Yee:Native:2009} and follow up work on
  web assembly sandboxing~\cite{Haas:Bringing:2017,
  WebAssemblyCommunity:Security:2020} allow unsafe third
  party (native) libraries to safely operate within the same
  address space as the application.
  %
  Recent research prototypes have shown efficient and
  powerful intra-address space
  isolation~\cite{Vahldiek-Oberwagner:ERIM:2019,
    Liu:Thwarting:2015, Hedayati:Hodor:2019,
    Park:libmpk:2019, Hsu:Enforcing:2016,
    Litton:Lightweight:2016, Bittau:Wedge:2008,
    Koning:No:2017, Chen:Shreds:2016,
    Dautenhahn:Nested:2015, Narayan:Retrofitting:2020,
    Kuznetsov:Code:2014, Carr:DataShield:2017,
  Vasilakis:Automated:2018, Sung:Intraunikernel:2020}.
  %
  Even leading hardware vendors and researchers alike have
  explored architectural support for intra-process
  separation~\cite{Zamyatin:Intel:2013, Intel:Control:2016,
    :Intel:2020, ARM:ARM:2001, IBMCorporation:Power:2017,
    Dahad:Arm:2019, Corbet:Memory:2015,
    Mogosanu:MicroStache:2018, Schrammel:Donky:2020,
    Song:HDFI:2016, Clements:Protecting:2017,
  Frassetto:IMIX:2018, Woodruff:CHERI:2014,
Watson:Cheri:2015, Du:XPC:2019}.

  \iffalse
  % --------------------
  The core problem is that operating systems do not have
  intra abstractions and therefore can't do it.
  %
  The goal of this work is create such a cross layer
  solution but do it only in userspace and without resorting
  to lower performance or lower compatibility solutions.
  %
  %While implementing in the kernel seems like the obvious choice, it brings
  %signficant complexity, which could leave gaps in protection just as is the
  %case with containerization, as such we believe a simpler abstraction layer
  %can be built at the system call api layer and done there.

  % --------------------
  The only meaningful way is to be independent and use the
  most efficient mechanism available.
  %
  The goal of this work is to maintain the benefits of
  recent intra-process isolation while making them more
  secure, and possibly enabling a new model for sandboxed
  applications.
  %
  The key idea is to virtualize all system calls so that a
  security monitor can add the intra-domain abstraction on
  top of the OS.
  %
  Thus adding a layer to deny violations of the simple high
  level isolation policies.

  % --------------------
  In this work we aim to provide a fast, compatible, and
  secure solution to intra-app isolation.
  %
  The core ides is to extend prior work with a new system
  call virtualization protection layer in userspace.
  %
  In this way, \system can filter bad operations that
  violate the security policy while allowing standard
  functionality.
  %

  %
  To this end we present a new intra-process separation
  architecture, \system.
  %
  The primary goal of \system is to insert a thin
  virtualization layer on top of the operating system so
  that system resources can be properly monitored for safe
  use.
  %
  Although this idea is similar to containerization, our
  approach retrofits it into existing processes so we can
  maintain high speed.
  %
  \fi
  % --------------------
  Single-address space separation minimizes costly context switches by using
  lightweight hardware and software protection mechanisms.
  %
  From early software only approaches like SFI and even early hardware
  approaches like SMTH, there is a continued struggle for fine-grained
  protection.
  %
  More recently, Provos \etal introduced the notion of \emph{privilege
  separation} that seeks to decompose a monolithic application so that
  least-privilege security policies can be enforced, but comes with the
  significant costs of programmability---manual object level code
  modification---and performance---address space isolation.
  %
  Fast-forward almost twenty years and we now have single-address space
  hardware~\cite{} and software~\cite{} innovations combining the goals of early
  research with retrofitting privilege separation into applications.
  %
  \fi

  % -------------------- intro intro 1.31.21 i like, but too high level
  Single-address space separation minimizes costly context switches by using
  lightweight hardware and software protection mechanisms.
  %
  From early software only approaches like SFI and even early hardware
  approaches like SMTH, there is a continued struggle for fine-grained
  protection.
  %
  More recently, Provos \etal introduced the notion of \emph{privilege
  separation} that seeks to decompose a monolithic application so that
  least-privilege security policies can be enforced, but comes with the
  significant costs of programmability---manual object level code
  modification---and performance---address space isolation.
  %
  Fast-forward almost twenty years and we now have single-address space
  hardware~\cite{} and software~\cite{} innovations combining the goals of early
  research with retrofitting privilege separation into applications.
  %


  The first insight is that \system forces all uses of system calls to go
  through the protected monitor.
  %
  The second insight is to use this forced control flow to insert the
  virtualization.
  %
  The basic rule of the virtualization is to deny all system calls that would
  allow the system call monitor to be bypassed, presenting a complementary
  security architecture to
  %which is coincidentally the same set of properties enforced by
  intra-process separation approaches~\cite{Vahldiek-Oberwagner:ERIM:2019,
  Hedayati:Hodor:2019, Schrammel:Donky:2020}.
  %
  Control is asserted by using a seccomp filter allowing \syscalls only from the
  security monitor, combined with a novel, protected call gate mechanism that
  uses a new lightweight \syscall instruction protection
  % capability
  scheme so that if the call gate is not used the instruction cannot be used.
  %
  %The core method is to nest the monitor into the runtime using a combination
  %of efficient memory isolation mechanisms along with a set of mechanisms
  %thwarting unmonitored execution of system calls by the untrusted portion.
  %
  The first is to force control-flow through the monitor without resorting to
  costly control-flow integrity mechanisms, which add an unnecessary
  overhead~\cite{Vahldiek-Oberwagner:ERIM:2019} while not being fully
  guaranteed~\cite{Evans:Missing:2015}.
  % Anjo: Its going to be hard to find this number, since it highly depends on
  % the fine-graines of the approach. I think for what we want this requires
  % only a very coarse CFI. Which is something Michael and I have been
  % suggesting based on CET.  So I'm not sure that we can use something ehere.
  % In erim we used the following sentence: (don't copy) "For example,
  % code-pointer integrity (CPI), one of the cheapest reasonably strong CFI
  % defenses, has a runtime overhead of at least 15% on the throughput of a
  % moderately performant web server (Apache) [31, Section 5.3]."
  %
  The second is to examine, understand, and derive policies that will keep
  memory isolation in place and avoid system call bypass attacks.
  %
  The third is to properly virtualize signals as they present subtle ways in
  which control flow and protection state can be corrupted.
  %
  The fourth is to inject the monitor without breaking existing state---by
  controlling signals the secure monitor must emulate complex functionality as
  well move the untrusted components out of the default domain expected by
  Linux.


\iffalse
  % -------------------- Motivate apps have bad stuff and
  %  aren't changing
  Today's application runtimes are complex and incorporate
  code from many disparate components.
  %
  For example, safe languages and web browsers interface
  with unsafe code or depend on libraries from untrustworthy
  sources~\cite{Qin:Understanding:2020}.
  %
  Whether due to bugs~\cite{Durumeric:Matter:2014,
  CVEMozilla:Security:2020, CVE:Rustlang:2020,
Qin:Understanding:2020} or directly malicious
code~\cite{Cimpanu:Two:2019, Karger:Limiting:1987,
Thompson:Reflections:1984, Yee:Native:2009}, applications
demand intra-app protection to remain trustworthy.
  % --- Introduce priv sep as the solution
  The standard method is to apply \emph{privilege
  separation} so that sensitive state is protected from
  leakage or corruption~\cite{Provos:Preventing:2003}.
  %
  Privilege separation has become so successful that almost
  all users rely on it daily---with native code sandboxing
  in production browsers since 2008~\cite{Yee:Native:2009}
  (Firefox, Chrome, IE, \etc) and OpenSSH since
  2003~\cite{Provos:Privilege:2003,
  Developers:OpenSSH:2020}---and even major hardware vendors
  (\eg \intel, Arm, \etc) and researchers alike are searching
  for the best intra-process protection
  mechanism~\cite{Grisenthwaite:Safer:2019,
    Woodruff:CHERI:2014, Watson:Cheri:2015, Du:XPC:2019,
    mpk, mpx, trustzone, sgx, vmfunc, iphone_secproc, etc.}.
  %

  % --------------------
  The core goal of \system is to preserve the efficient
  isolation presented by recent intra-process isolation
  mechanisms while making them secure and not losing
  compatibility.
  %
  There are several methods by which to do this.
  %
  In this section we first introduce the basic idea of
  privilege separation and then explore alternative ways to
  apply privilege separation and comment on their
  suitability relative to our goals.
  %
  \fi

  \iffalse
  % NDD: I don't think we need an example but maybe add later
  %%--------------------------------------------------------
  \paragraph{Motivating Example}
  %%--------------------------------------------------------
    Do we need an example to motivate the fine grained
    stuff? Are we prepared to implement it.
  %
  \fi

    % --------------------
    The basic idea is to partition an application so that
    code and data are isolated.
    %
    The terminology has been used in several ways and to
    simplify we describe our notion of privilege separation
    as being one of the following: 1) sandbox
    untrustworthy/buggy code (standard V8, native client
    iso, wasm), 2) provide exclusive access to sensitive
    data to a small trusted monitor (priv sep, openssh,
    \ldots), or 3) compartmentalization with multiple
    domains having exclusive access to their own private
    data (\ldots).
    %
    The model is to treat code as subjects and data as
    objects (fitting Lampson's access control matrix), where
    the privileges are: call, return, read, write, alloc,
    and free.
    %
    The basic guarantees are that the protection system will
    enforce these policies by separating the application
    into distinct domains and protecting objects using the
    mechanisms.
    %
    The key issue is separating the system while improving
    security but minimizing performance costs.

  %%--------------------------------------------------------
  \paragraph{In the OS}
  %%--------------------------------------------------------

    % --------------------
    The most sensible mechanism to enforce privilege
    separation is the operating system.
    %


    most sensibly provided by separating a
    subset of code and data into a separate address-spaces
    and using IPC for
    sharing~\cite{sgx,trustzone,eptvmfunc,lwc,provos,etc}
    (as depicted in Figure~\ref{fig:problem}).
    %The most prevalent approach separates components into
    %distinct address-spaces~\cite{}, transforming
    %control-flow and data access into process level IPC.
    %
    Unfortunately, address-space separation is slow and
    cannot handle applications with frequent
    interactions~\cite{}, which are beginning to dominate
    certain markets (\eg cloud serverless compute
    V8~\cite{fidnme} and secret leakage~\cite{findme}).

    % --------------------
    It would seem then that the only solution would be to
    modify the OS abstractions, which many have done to great
    effect.
    %
    Unfortunately, the Linux community does not care about
    this abstraction---several important LSM patches have been
    halted, something else, and something else.
    %
    Alternatively, a TEE or VMM based, but these technique add
    more layers and remain slower than new lightweight is
    abstractions.

  %%--------------------------------------------------------
  \paragraph{Below the OS}
  %%--------------------------------------------------------
    \review{this section is just a dump of other junk}

    % --------------------
    List: donkey, microstache, ept, sgx, tz, keystone
    (risc-v), imix, mine references from donkey paper,
    \ldots
    %
    Maybe just want to focus it on actual intra-priv sep
    systems not just mechanisms that do it\ldots ie don't
    include MPK\ldots

    % --------------------
    Instead of integrating the abstraction into the OS and
    using address space separation, many efforts seek to use
    lower layers to provide intra-app isolation.
    %
    While they address the issue of memory access through
    system calls they do not solve\ldots
    %
    Donkey, is unique in that it is going below the
    OS\ndd{wait does donkey not go below the OS?}. Does
    Microstache not go below the OS? In some way the
    protection mechanisms are hardware based but they
    actually are controllable by the OS and therefore the OS
    would still allow access\ldots or maybe in microstache
    it would still hold true? I think it would, but the OS
    still controls the regs? \ldots Well by default I think
    the hardware would enforce the iso unless changed by the
    OS and therefore no syscall bypass\ldots but this is an
    ``accidental default'' not an enforced property, and we
    didn't implement the OS, so who knows what it would do
    and what things we might break.

  %%--------------------------------------------------------
  \paragraph{On top of the OS: Nested Intra-Privilege
  Separation}
  %%--------------------------------------------------------

    \review{this section is just a dump of other junk}

    % --------------------
    Recent work has sought to \emph{nest} a security monitor
    into the runtime environment with lightweight isolation.
    %
    In contrast to heavyweight and slow processes or fast but
    restrictive sandoxing, nesting monitors can support each
    of the privilege separation use cases while enforcing
    least-privilege which puts the most pressure on the
    runtime mechanism.
    %
    Several recent works do so to great effect.
    %
    ERIM, HODOR, \ldots.
    %
    Unfortunately, each of these techniques suffers from one
    main drawback---they are easily bypassable through the
    system call interface.
    %

    % --------------------
    %\paroutline{Gap}{they have problems though}
    %
    In spite of this success, approaches for retrofitting
    fine-grained privilege separation into general
    applications are lacking.
    %
    Sandboxing efficiently isolates native code by using SFI
    to restrict control-flow, memory, and system call
    access~\cite{Wahbe:Efficient:1993, Yee:Native:2009,
    Narayan:Retrofitting:2020}---depicted in
    Figure~\ref{fig:problem}---but without system calls it
    cannot support general purpose privilege separation,
    missing threats such as
    HeartBleed~\cite{Durumeric:Matter:2014}.
    %
    Alternatively, several approaches split applications into
    multiple parts and separate them with
    processes~\cite{breakapp,\ldots,\ldots}.
    %
    These approaches have been successfully deployed, \eg
    OpenSSH~\cite{privtrans, separatedssh}, however, process
    isolation is heavyweight in terms of transformation effort
    and runtime performance.


    % --------------------
    In contrast, recent work has taken to
    nesting~\cite{Dautenhahn:Nested:2015} a thin monitor into
    the execution environment that provides control and data
    isolation of the trusted component at a fraction of the
    cost.
    %
    There are many such applications, two of the most
    significant are exclusive protection of certain
    secrets~\cite{} and the rise of the \emph{safe region}
    paradigm that is used to add safety properties to the
    unsafe code.
    %
    While these are powerful, a recent attack demonstrated a
    fundamental flaw in the threat model---an attacker can use
    the OS abstractions/objects to bypass the security
    monitor.
    %
    The reason is that intra-proccess domain abstractions are
    invisible to the OS and therefore not respected.
    %
    For example, a \Code{k}
    %
    Their main problem is that they only consider memory and
    not system

    % --------------------
    While the goal of this work is to enable an existing
    abstraction to work, we reuse and extend it.
    % ---- S/NS explained
    The basic model for this work is to have a secure nonsecure
    world split.
    % ---- Work aiming and doing this
    Many efforts do this, trustzone, erim, etc... privsep ssl
    % ---- Spectrum: exclusive or sandbox
    The key feature is to enable the protection of a small
    subset of data or the sandboxing of an untrusted pieces of
    code.


    \review{link to related work table to show the
    gaps}\ndd{need to focus on the right criteria}


    % --------------------
    One of the biggest challenges in privilege separation is
    dealing with the contrasting goals of least-privilege
    and efficiency.
    %
    Least-privilege suggest fine-grained minimal privileges
    but that requires higher costs for cross-domain
    interactions.
    %
    Thus, regardless of the particular policy, as long as
    there is communication, the mechanism plays a
    significant role in the viability of any approach.

    %

    % --------------------
    In contrast, recent work has taken to
    nesting~\cite{Dautenhahn:Nested:2015} a thin monitor
    into the execution environment that provides control and
    data isolation of the trusted component at a fraction of
    the cost.
    %
    In essence, nested monitors apply privilege separation
    of the application into a \emph{\td} and \emph{\ud},
    where monitor code and data are protected from \ud
    access.
    %
    There have been many such systems, and the most relevant
    distinction from \system is the mechanism used to gain
    separation, as none of them provide sufficient
    in-process system call protection for the monitor split.


\if 0
% --------------------
\subsubsection{Fangfei's Original Section on syscall nexpoline}
% --------------------

However, even we control the loading of untrusted code, in the runtime it may still break the third policy.

A general idea is self-modifying code, the executable code
contains \wrpkru, but it can dynamically modify itself to generate
such instruction bytes.

To prevent this, we can conduct another policy: we must scan any modification towards executable pages before it can be executed.
For efficient consideration, we created a restricted version of this policy: all modification towards executable pages must be
explicitly committed through our trusted monitor. In practices, this means all pages are $W\oplus X$.
So untrusted code needs first remove the executable privilege of pages to be able to write, then mark it as executable
but not writable to execute them.

Because kernel and CPU is totally unaware of our policy, the policy may be breaked when untrusted code interacting with system calls.
To achieve the protection, we need to also change some behaviours of certain system calls.
Ptrace has been widely used in such protection to sanitizer syscalls, % add ref
but it has a nonnegligible overhead since either all syscalls must be sent to another security monitor running in a dedicated process space,
or in other apporches, a seccomp filter is used to filter out non-sensitive syscalls while other syscalls still need to be sent to another
process. And, although the tracer process can modify the running state of tracee, all modification happens remotely and causes more overhead.

Our new solution based on the new privilege is \emph{system call virtualization}. We patched all syscall instructions in glibc and changed them into
a call to {\tt syscall\_trap} function in trusted code. It switches into trusted domain and virtualize the syscall.

By virtualizing, we can have a function that acts as the kernel and invoke the real syscalls to achieve the same features while maintain our policy.
The fact that we are in the same process space provides more flexibility on invoking the syscall, because from the view of the kernel we are still
the same process. This allows us to use complex policies and local datastructures without introducing extra overhead.

For example, {\tt mmap} is a syscall that creates a new mapping in our memory space. We enforced our policies in our {\tt syscall\_trap} by checking
its arguments and prevent it from mapping on our trusted memory or creating executable pages that contains WRPKRU instruction. And, we change its
protection key so the untrusted code can read or write on these memory.

If we are using ptrace, the arguments check is roughly the same, but to inspect the mapped pages with ERIM, we must also mapping the same pages in
our monitor process. To change the memory protection key, we need few times of context switching between the two processes so we can invoke that syscall
in that process space and recover the context for it. With our syscall virtualization, it is a normal code running inside trusted domain.

%For example {\tt mprotect}, this system call changes the protection properties on memory pages. It can make a writable page executable.
%We redirect all system call from glibc to our trusted code entrypoint. In our code, we inspect the arguments to enfore $W\oplus X$, and also
%ERIM scan. And, we prevent our trusted pages from being touch by this system call so untrusted code cannot modify anything on them.

%Although kernel is exptected to maintain such policy while providing kernel services, only syscalls that directly read or write the userspace
%memory with interface like copy(from|to)user that takes userspace's memory protecetion into account can prevent kernel from breaking MPK.

%Some system calls have been known to allow read or write to process memory (add ref).
%This further require us to also filter other sensitive system calls that are not directly changing the userspace memory. According to (ref),
%this mainly contains file based system calls. Linux has a special file called \/proc\/self\/mem, by reading this file with an offset, we are
%actually raeding the real userspace memory of that address while bypassing all MPK and memory protection.
%We filtered all file descriptors backed system calls so all read/write on this particualr file.

We virtualized some of the Linux syscalls while pass-throughed the others.
Within the virtualized syscalls, most of them are filesystem related.
That is because Linux has a procfs that allows program to read or write other process's memory space with a file descriptor including the process itself.
Although kernel respect MPK settings in most syscalls, these syscalls are exceptions which only check the normal page based protection. % addref
Our virtualized syscalls trace all opened file descriptors to {\tt /proc/self/mem} and reject any reading or writing to trusted memory.

We virtualized memory related syscalls to record all pages mapped in userspace and the protection attribution, especially the pages used in trusted domain.
So our trusted memory will not be accidently unmap or remap by the kernel, and any pages created or
promoted as executable will be scanned by ERIM and $W\oplus X$ enforced. This record is also used by filesystem related syscall to prevent bypassing through
procfs.

The $W\oplus X$ restriction is tricky because Linux supports many ways of sharing physical pages acrossing system. We cannot allow one page to be both
writable and executable, but we also need to prevent two pages to be mapped into one shared physical memory while one of them is writable and another
is executable. To ensure this, we created a speical attribution for memories that have only been mapped once but not executable: retired, and we only allow
retired pages to be promoted as executable. The relationship among attributions is shown in \ref{fig:attr_rel}. Beside that, when creating a executable map
to file descriptor, we will not use the original syscall which might create a map that shares \emph{copy-on-write} pages with other mapping,
instead, we create a private map and read the file and scan it with ERIM.

The mechanism for system call virtualization requires our final policy: all sensitive system calls must from trusted domain.
By using seccomp filter, we installed a policy that ensures all sensitive system calls have a PC that laid inside trusted code.
The tricky thing here is that an attacker can jump to our syscall instruction directly
since MPK does not prevent code from executing even the current PKRU says you cannot access the code.
So, from the seccmop perspective the system call comes from trusted code but it is actually not.

To alleviate this, we used a randmoized trampoline to hold our system call secquence as shown in \ref{fig:trampoline}.
We reserve multiple pages of executable memory in trusted domain. These memory cannot be read from untrusted domain.
And we put a policy in seccomp filter that we only allow syscalls come from this range of the memory address.

% Randomized figure but remove for now
\iffalse
\input{figs/rnexpoline}
\fi

These pages are filled with {\tt 0xCC} which is {\tt int3} in x86. And, we put one {\tt syscall; ret} sequence inside this address space.
We save the address to syscall instruction in a linker selected address in the trusted domain.
Any syscalls inside trusted domain would be a reading of the trampoline address from this memory to register and call directly to it.

Because the protected memory is not readable from untrusted domain, to execute such read, the control-flow must from the trusted entrypoint
and thus it serves as a domain checker and only trusted domain can execute the syscall. The read address is the key to run system call instruction.

To prevent the address leaking, we re-randomize the trampoline routinely after executing the system calls.
However, we could configure the size of the trampoline pages and the frequency of the re-randomization, therefore the security and performance can be efficiently configured.
The probability of the successful random guess attack could be described as follows.
\begin{equation}
P = 2\frac{Randomize_frequncy} {Pagesize \times Pagecount}
\end{equation}
For example, if we reserve 16 pages for the trampoline, and we re-randomize every 32 syscall execution, the probability will be 1/1024.
\fi



% --------------------
THIS IS THE old nested execution subsection. Throwing here because i've got
stuff all over and want to make surei t doesn't dissapear as we are repurposing
the model.tex for the priv sep model.


  % --------------------
  \arch is a userlevel intra-process separation
  architecture, but unlike prior efforts we provide a more
  complete set of objects to protect along with support for
  facilitating client applications.
  %
  Our challenge is to insert the security monitor into the
  application's runtime and represent all system objects to
  deny malicious information and control flows without being
  slower than ptrace, which simulates state of the art
  multi-process privilege separation approaches.
  %
  Not only does \arch prevent attacks on the monitor
  isolation itself, it can also enable a unique class of
  efficient multi-principle, sub-process system object
  policies.
  %
  We break the key elements of \arch into three classes: 1)
  the privilege model, 2) the architecture definition and
  associated policies, and 3) interface for facilitating app
  compartmentalization.


%%----------------------------------------------------------
\section{Nested Execution Environment Approach}
%
\label{sec:model}
%%----------------------------------------------------------

  % --------------------
  \begin{figure*}[]
      %
      \begin{center}
        \includegraphics[width=\textwidth]{figs/arch}
      \end{center}
      %
      \caption{\label{fig:sysarch}
        %
        \system Architecture.
        %
      }
  %
  \end{figure*}

 % \input{priv-tbl}

\iffalse
  % --------------------
  The fundamental goal of \system is to preserve the
  integrity of the nested security monitor within
  intra-separation systems.
  %
  This is a different objective than the protection systems
  themselves, which have diverse abstractions from exclusive
  access to sandboxing.
  %
  We then specialize a set of security properties that must
  be in place given the specific mechanisms we've chosen and
  perform a systematic analysis of all system calls to
  identify sensitive and non-sensitive operations.
  %
  After that we define a set of policies that must be
  enforced in order to uphold the high level security
  property.
  %
  The overall theme of the description in this section is to
  specify a base configuration of the system which adheres
  to an initially secure system and then to identify the set
  of transition relations that can change the configuration,
  and to establish rules for each transition so that the
  system will always maintain a safe state.

\fi


  % --------------------
  \system is a userlevel intra-privilege separation
  framework, but unlike prior efforts it emphasizes full
  virtualization of system calls and signals.
  %
  Our challenge is to insert the security monitor into the
  application's runtime and ensure all \syscall uses go
  through \system and signals are properly virtualized
  without being slower than ptrace.
  %
  By doing this, \system is able to assert any policy and
  emulate access to system resources while ensuring monitor
  isolation.
  %
  In this section we provide an overview of the approach,
  define the properties and policies required for a
  privilege separated nested execution environment, and
  describe the design philosophy.

  % --------------------
  \input{principles}

  % --------------------
  \subsection{Overview}
  % --------------------

  \label{sec:design-overview}

  \iffalse
  % --------------------
  Our approach is to combine prior work on nested execution
  monitor isolation with new techniques to eliminate threats
  from signals and system calls.
  %
  The result is a new privilege separation framework that
  virtualizes all system calls and signals by inserting a
  monitor and emulating.
  %
  By doing this \system is able to assert any policy it
  desires, \eg deny all, allow subset, allow but deny some
  functionality.
  %
  As indicated, ptrace could do this but would result in a
  prohibitively slower mechanism.
  %
  Instead, we nest the monitor within the process
  itself and provide a set of properties with four
  separate mechanisms as depicted in
  Figure~\ref{fig:sysarch}.
  % --------------------
  \fi

  % --------------------
  \system injects the monitor into the application, as the
  \td, and removes the ability of the \ud to directly modify
  \emph{privileged state}.
  %
  Privileged state includes: protection information (\eg
  protection control (like MPK or access control policies),
  code, monitor code and data, direct system call
  invocation, raw signal handler data, and monitor
  control-flow).
  %
  The monitor is inserted on startup by hooking all system
  call execution and initializing the protection state so
  that the monitor is isolated with no files opened or
  mapped.
  %
  There are three major subsystems in \system that are each
  dependent on the others to maintain isolation: privilege
  (memory), syscall, and signal virtualization.

  % --------------------
  \paragraph{Privilege and Memory Separation}
  partitions the application into two spaces, \td and \ud,
  and uses \wrpkru to switch between the two domains, which
  changes the accessible set of memory.
  %
  Access to \wrpkru instructions for malicious uses is
  prevented by using a technique we call \emph{instruction
  capabilities}.
  %
  The primary requirement of privilege virtualization is to
  \emph{ensure the \ud does not gain control of execution
  while in the \td mode.}
  %\begin{prop} ensure monitor state remains isolated (not
  %accessible or corruptible) from the \ud.  \end{prop}

  % --------------------
  \paragraph{System Call Virtualization} ensures that all
  \syscalls are only executed by \td and additionally
  supports any combination of none, partial, and unmodified
  \syscall support by using instruction capabilities.
  %is provided by a technique forcing all \syscall
  %operations through the monitor, again using instruction
  %capapbilities to ensure the \ud cannot invoke one
  %directly.
  %
  %System call virtualization asserts two key requirements:
  %
  %\begin{prop} only the monitor can invoke \syscall
  %instructions \end{prop}
  %%
  %\begin{prop} prevent monitor isolation bypass through
  %system interfaces \end{prop}
  %%
  The challenge is stopping the \ud from
  generating/injecting its own syscall instruction or
  finding unintended ones. CPI blocks access to unintended
  syscall instructions but that would add a substantial performance
  cost to the system.
  %
  Instruction capabilities operate similarly protection
  rings where the \ud is denied use of the instructions using
  any combination of language based security mechanisms.
  %
  \system uses its control over \syscalls to ensure that \td
  memory is never made accessible to the \ud through system call
  resources.
  %

  % --------------------
  \paragraph{Signal virtualization} is achieved by setting
  up a virtual signal queue in \system that effectively
  replicates what the kernel is doing.
  %
  Securely managing signals turns out to be one of the
  biggest challenges because the virtualization technique
  opens up a small interface that could be used to attack
  \system as well as demands complex concurrency control.
  %
  Signal virtualization ensures that raw signal handler
  and CPU state are not accessible to the \ud, which could be
  corrupted to manipulate memory protection policies or
  control-flow of \td, and that all signals are handled
  atomically to avoid corruption of \system runtime.
  %
  %\begin{prop}
  %%
  %1) prevent corruption of privilege CPU state accessible
  %to handlers (\ie \pkru value),
  %%
  %\end{prop}
  %%
  %\begin{prop}
  %%
  %2) prevent atomicity violations that would lead to \ud
  %gaining control while in \td context, and
  %%
  %\end{prop}
  %%
  %\begin{prop} 3) intercept faked signals that are a
  %byproduct of virtualizing signals in usermode.
  %%
  %\end{prop}

  % --------------------
  \paragraph{Nested Monitor Property}
  %
  \label{sec:nestedprop}
  % --------------------

    % --------------------
    We provide the following informal description of a high
    level property and a set of invariants that ensure the
    property.
    %
    The basic property is that:
    %
    \begin{prop}
    %
    Privilege Separation Integrity: All privileged bits,
    whether CPU register state or memory, cannot be modified
    or accessed by the \ud.
    %
    \end{prop}
    %
    Care must be taken when attempting to break down the
    properties because the nested model makes certain state
    accessible---in contrast to traditional ring-based
    protection models.
    %
    In a sense, these properties ensure a virtual protection
    ring within the process and address space.
    %
    Our method for describing correctness is inductive: the
    system starts in a state where the \td and \ud are separated
    and all protection bits are in place.
    %
    We then ensure that the following invariants hold true:
    %
    %To derive this set of invariants we combine PKU
    %Pitfalls as well as our own invariants.
    %
    %The high level property can only be achieved when the
    %following are
    %
    \begin{inv} Direct Access Integrity:
      %
      \label{inv:memiso}
    %
    \ud never executes while \pkru is in \td in context.
    %
    \end{inv}
    %
    \begin{inv} Code Execution Integrity:
      %
      \label{inv:codeexec}
    %
    All \ud code is validated prior to being mapped $W
    \oplus X$.
    %
    \end{inv}
    %
    %\begin{inv} Guaranteed Mediation or Protected Call
    %Gates:\end{inv}
    %
    \begin{inv} Syscall Execution Integrity:
      %
      \label{inv:sysexec}
    %
    Prevent \ud from directly executing \syscall.
    %
    \end{inv}
    %
    %\begin{inv} Indirect Access Integrity:
    %%
    %As previously indicated, \syscalls allow memory access
    %through many kernel interfaces, all need to be denied.
    %
    \begin{inv} Protection Context Integrity:
      %
      \label{inv:mapping}
    %
    Trusted domain memory never mapped into the \ud context.
    %
    \end{inv}
    %
    \begin{inv} \syscall Access Integrity:
      %
      \label{inv:iaccess}
    %
    Access through sudo filesystems (procfs) is denied.
    %
    \end{inv}
    %
    \begin{inv} Atomicity of Monitor:
      %
      \label{inv:atomic}
    %
    Trusted domain operates atomically from the perspective of the \ud.
    %
    \end{inv}
    %
    %% Like this but didn't fit yet
    %%\begin{inv} Monitor Exit Integrity:
    %%
    %Control never leaves the monitor without going through
    %exit gate, which is essential as signal virtualization
    %%adds an interface to spoof signals which can influence
    %%control in the monitor.
    %%
    %\end{inv}
    %
    \begin{inv} Signal Handler Integrity:
      %
      \label{inv:sigintegrity}
    %
    Signal handler context is not directly modifiable or
    influenced by \ud.
    %
    \end{inv}

  \iffalse
  %
  The basic properties enforced:
  %
  \begin{prop} Nested Monitor Integrity\end{prop}
  %
  \begin{prop} Syscall Virtualization\end{prop}
  %
  \begin{prop} Signal Virtualization\end{prop}
  %
  Direct monitor integrity is enforced using MPK based
  isolation (as explored by ERIM/Hodor/etc).
  %
  Due to the complexity of the system interface, the
  monitors isolation depends on both system call and signal
  virtualization.
  %
  Syscall virtualization is achieved through a monitor that
  removes the ability of the \ud to execute a system call
  directly, forcing all calls through the monitor.
  %
  Specifically, we introduce a new mechanism that uses
  seccomp to restrict system call execution to a small
  region of memory and then use randomization to locate the
  instruction.
  %
  %\system forces system call control by using a simple
  %seccomp filter, however, because \system is nested in the
  %address space and we must be able to execute \syscall
  %without first transitioning to the kernel, we need to
  %leave it mapped into the address space.
  %%
  %This means that its location could be identified and then
  %directly executed by the \ud.
  %%
  %Thus we must ensure that such a control flow cannot
  %happen, which we solve with a new lightweight instruction
  %randomization technique.
  %
  Signals can expose low-level protection state (\pkru) and
  also generate subtle control flow behavior that if left
  unchecked could allow the \ud to gain control while memory
  permissions are set for the \td.
  %

  \fi


\iffalse
  %
  System asserts isolation by ensuring each modification or
  transition to protected operations does not invalidate the
  following properties:
  %
  \begin{prop} Monitor Access Integrity:\end{prop} while the \ud
  is executing all monitor state is protected from read and
  writes.
  %
  %\begin{prop} Guaranteed Mediation or Protected Call
  %Gates:\end{prop}
  %
  \begin{prop} Monitor Control Integrity: privilege state
    can only be modified if the monitor is entered through a
    protected call gate, ensuring that all protection
    policies are asserted.  \end{prop}
  %
  \begin{prop}Syscall Execution Integrity:
  %
  prevent \ud from directly executing \syscall. The
  challenge is stopping the \ud from generating/injecting
  it's own syscall instruction or finding unaligned ones.
  Could solve this with CPI but that would add an automatic
  high performance cost to the system. Can we do it more
  economically?
  %
  \end{prop}
  %
  \begin{prop} System Bypass Integrity:\end{prop}
  %
  \begin{prop} Signal Virtualization and
    Integrity:\end{prop}
  %
  \begin{prop} Direct Memory Protection:\end{prop}
  %
  \begin{prop} Atomic Monitor:\end{prop}
  %
  \begin{prop} Monitor Exit Integrity:\end{prop}  Control
  never leaves the monitor without going through exit gate:

  % --------------------
  \system forces control using a simple seccomp filter,
  however, because \system is nested in the address space
  and we must be able to execute \syscall without first
  transitioning to the kernel, we need to leave it mapped
  into the address space.
  %
  This means that its location could be identified and then
  directly executed by the \ud.
  %
  Thus we must ensure that such a control flow cannot
  happen, which we solve with a new lightweight instruction
  randomization technique.
  %
  \system ensures that it's runtime is protected from
  compromise by using MPK based single-privilege level
  virtualization as introduced by ERIM.
  % --------------------
  %Nesting and virtualizing privilege creates unique
  %challenges for system call virtualization, the obvious
  %being to 1) ensure system calls only originate from the
  %\td and  2) \td state is protected.
  %%
  %Less obviously, \system must isolate the monitor from
  %access through system objects and signal abuse, both of
  %which can influence data layout, access control policies
  %for memory regions, and control flow.
  %
  As indicated, protection of the monitor also depends on
  proper isolation from indirect attack through system calls
  and signals.
  %
  Signals turn out to add the most complexity as
  virtualizing them create unique corner cases that an
  attacker might be able to abuse.
  %
  %To isolate the monitor, we must protect against three
  %main classes of attack: 1) direct memory and control-flow
  %protection, 2) memory access through system calls, and 3)
  %memory and non-control data attacks through signal
  %manipulation.

  \fi

  % --------------------
  %\subsection{Privileges}
  % --------------------
  %The privileges in our system include access to: syscall
  %instruction, PKRU regs, alias control, etc.


  % --------------------
  %\subsection{Privileges: Objects to Protect}
  % --------------------
  %  Privileges: What are we protecting and why?

  % --------------------
  %\subsection{Attacks}
  % --------------------
  %- Attacks: How to compromise and classification?

  % --------------------
  %\subsection{New Attack Vectors}
  % --------------------
  %- Syscall Attack Vectors
  %- Signal Attack Vectors

%%%%% TODO
\iffalse %TODO flessh it out
    % --------------------
    Unfortunately, despite the sophisticated and working
    machinery, Linux/POSIX provides interfaces through
    kernel objects that allow the basic property to be
    bypassed.
    %
    PKRU Pitfalls paper did some analysis to expose this
    class of threats and we briefly summarize here, as they
    lay the foundation to \system design as well as a few
    new attacks we expose in this work.

    \writeme{Fill this out in five ish subsections}

    %%--------------------------------------------------------
    \paragraph{}
    % --------------------

\fi

\iffalse
  % --------------------
  \subsection{Security Policies}
  % --------------------

    % --------------------
    \paragraph{Alias Integrity}
    %
    As prior work on intra-privilege virtualization noted, a
    key aspect of protection for intra-level separation is
    that protection is typically enforced on the mappings
    between virtual and physical resources.
    %
    The whole idea of virtualization is built on this fact,
    therefore, any policy or alias that might insert a new
    unmediated access edge must be protected against.
    %
    Of course building security into (modify Linux like
    lwcs) or below the OS (virtualization hardware, or like
    more recent Donky hardware that enables user level
    monitor isolation), however, the high level property
    remains the same.

    % --------------------
    \paragraph{Mapping Policies}
    %

    % --------------------
    \paragraph{\syscall Instruction Capabilities}
    %
    Unlike the \wrpkru instruction that is long enough to be
    removable from the runtime, \syscall is a \review{2}
    byte sequence and not as easily removed, given many
    false positives.
    %
    As such we needed to devise an alternative method for
    ensure this property.

    % --------------------
    \paragraph{Signal Protections}
    %

    \fi


==> avail.tex <==
%-------------------------------------------------------------------------------
\section*{Availability}
%-------------------------------------------------------------------------------

USENIX program committees give extra points to submissions that are
backed by artifacts that are publicly available. If you made your code
or data available, it's worth mentioning this fact in a dedicated
section.


==> cet-bg.tex <==
Briefly, CET guarantees a shadow stack (returns return to the caller) and
indirect jump can only target locations that are prefaced with end branch
instruction.  
%
To achieve this, it adds an ENDBR64/32 instructions and a shadow stack as a
trusted source of the stack. 
%
Beside, it also support a legacy bitmap to mark all pages that can bypass the
indirect jump tracking, but the shadow stack must be used across the whole
application.  
%
Although Intel is promptly supporting CET in latest kernel and glibc, its still
incomplete so we made our own kernel patch and glibc modification to fully
utilize CET's features, especailly legacy bitmap so applications that are not
compiled for CET can still use \system.  


==> clone.tex <==
% --------------------
\subsubsection{\clone}
%
\label{sec:clone}
\todo{remove me}
% --------------------

  % --------------------
  Due to the diverse array of mechanisms and memory virtualization demands, we
  must specially deal with \clone and \fork.



==> disc.tex <==
%%----------------------------------------------------------
\section{Discussion and Future Work}
%%----------------------------------------------------------

  % --------------------
  Our results are very exciting, and in this section we
  discuss key aspects, highlighting potential for impact and
  value, and then conclude with future extensions.



==> domstruct.tex <==
  % --------------------
  A \domain is comprised of a set of capabilities:
  %
\begin{lstlisting}[language=C,style=customc]
struct segment {
  uint64_t sbegin;
  uint64_t send;
}
struct entrypoints {
  LIST_HEAD(list);
  uintptr_t next;
  uintptr_t prev;
}
struct segments {
  struct segment cs;
  struct segment ds;
  struct segment heap;
  struct segment stack;
}
struct pt_regs{
  uint64_t pc;
  uint64_t sp;
  ..
}
struct syscall_caps{ // something on specifying syscals }
struct signal_caps{ // something on specifying signal capabilities }
struct domain {
  LIST(entrypts);
  struct segments mem_segs;
  struct syscall_caps syscall_caps;
  struct signal_caps sigcaps;
  struct inst_caps instcaps;
  struct pt_regs;
}
\end{lstlisting}


==> erim-des-ff.tex <==

%%%%%%%%%%%%%%%%
%%% FIXME: I'm not familar with ERIM but I think large part of 
%%% this section is talking about ERIM.
%%% So, please fix this section if you are familar with it!!!!!
%%%%%%%%%%%%%%%%
% sounds like generating set?
Our goal is to have two major execution domains, one is trusted and another is untrusted. The propose of trusted domain is to keep the integrity(?)
of itself with MPK and some kernel features. 

MPK gives all memory pages a new property called protection key. And with a single instruction we can decide if current code can read or write on memory pages 
with specific protection key. 
We protect intravirt code and data by nesting them inside a special domain that other parts of the program cannot read or modify and put all MPK related 
operation inside the protected code. We call the protected code \emph{trusted code} and the related data \emph{trusted data}.
MPK cannot modify the executability of memory pages although it supports executable only by disabling both write and access on that page.
Because of that, we cannot prevent untrusted code using a jump instruction to arbitrarily jump into our code. 

However, we can use this feature to achieve a control-flow integrity policy: the WRPKRU instruction that switch MPK domain and grant 
read/write permission to trusted data. By accessing trusted data, we can test if our control-flow initiated from any WRPKRU instruction. 
And by checking the written PKRU value immediately after any MPK switching, this provides the adequate protection to our control-flow.

As a result, even an attacker jump into our code, the best thing they can achieve is they could execute these code as if they were executing them
inside untrusted domain without any privilege. Thus, our trusted data remains protected. Or, they might try to utilize our WRPKRU instruction since
that instruction does not require any privilege. But we can detect any uninteded MPK value because we verified it immediately after the setting. 
And any meaningful execution of trusted code that modifies trusted data will always passthrough our WRPKRU instruction, as long as we make sure we do 
not transfer our control-flow to untrusted code. 

We need our policy to be self-sustaining: there should not be any executable code which overrides MPK tags of trusted memory
or the PKRU register to trusted beside our entrypoints. 

From now, we starts to create a new privilege level that distinguished by PKRU register inside userspace applications. 
We call this new execution environment \emph{trusted domain} and the ordinary environment \emph{untrusted domain}.
Observing the meaning of WRPKRU here, we call it \emph{domain switching}. 

To summarize, we have the following core properties that establishes our userspace privilege system. 
\begin{enumerate}
  \item Set PRRU to trust domain in trusted code mark the entrypoint of trusted domain
  \item All control flows that leave trusted code must set PRKU back to untrusted
  \item Executable set PKRU instruction can only exist inside trusted code
\end{enumerate}

The first two policies can be achieved statically when generating our trusted code. 
And the third policy can initially achieved by scanning all untrusted code with ERIM. 



==> esyscall.tex <==

  % --------------------
  \paragraph{Signals for Ephemeral Syscall Trampoline}
  % --------------------
  Typically, an application returns via the {\tt sigreturn} system call.
  %
  In the case of ephemeral \nexpoline, we cannot rely on the kernel to return
  from a signal since we have to remove the \sysretg after the {\tt sigreturn}.
  %
  There are two cases: 1) a signal is delivered before the \syscall has finished
  and 2) the signal is delivered during the \nexpoline cleanup.
  %
  Hence, emulating {\tt sigreturn} in userspace is easier, especially since the
  x86 instruction set provides {\tt xrstor} instructions to load the CPU state
  from a memory location.

  % --------------------
  A signal delivered while cleaning up the \nexpoline creates a race condition.
  %
  To overcome this issue, we created a `transaction' for the cleanup phase of a
  system call.
  %
  If a signal occurs within the cleanup procedure, \system does not resume to
  the trap source, but rather to the start of the cleanup phase.
  %
  Therefore, we reset the {\tt rip} to the beginning of the cleanup phase and
  try to restore the signal context.
  %
  This procedure guarantees that signals occurring at any point within the
  \monitor clear the \sysretg.

  \if 0
  % too much detail noone knows what erim_regs are :D
  We cannot direct deliver to signal to user now because that requires a {\tt sigreturn}
  to the user directly. But, we can create an {\tt erim\_regs} above the signal stack
  and use {\tt sigreturn} to jump to the exiting code of {\tt syscall\_trap} which is exactly
  the beginning of the transaction we just described.
  In other words, we turn the signal delivering into a return from a syscall although the syscall
  itself does not exist. We set the register values in {\tt erim\_regs} to the values we need
  for untrusted signal handler. This is the same mechanism we used for delivering a signal
  after syscall although we do not have a syscall from user now. Then, the {\tt sigreturn}
  will bring us to the exiting transaction and eventually jump to untrusted signal handler.
  To be notice, here we could create a special code snippet for {\tt sigreturn}, so we would
  not reuse the {\tt syscall\_trap}'s code. We choose this because then we do not need to
  create another transaction area, and we can concentrate the code path that leave trusted domain
  into this one transaction and reduce the chance for anything go wrong. This will alter the
  state transaction model in \ref{fig:state} because now we are not directly return from Sig UT
  but go through T state with the assist of {\tt sigreturn}.

  This also prevent us from using {\tt sigreturn} for virtualized {\tt sigreturn} for the same
  reason. In this case, we will do something similar to direct signal deliver in signal handler.

  But, because we are in {\tt syscall\_trap} instead of a signal, we are not worried that
  {\tt syscall\_trap} will be re-entered anyone (user is pending, kernel will not deliver signal to syscall\_trap
  and syscall\_trap will jump to the syscall\_trap exiting code only if we are in untrusted domain).
  This allows us to unmask signal with {\tt sigprocmask} inside syscall virtualization.
  We use {\tt xrstor} instruction to restore fpu states. The PKRU value in xstate has been
  override with trusted to keep us inside trusted domain.

  Finally, we copy register values from {\tt sigframe} indicated by untrusted {\tt rsp} and, we retrieve
  the previous {\tt rsp} from {\tt sigframe}. We then allocate an {\tt erim\_regs} on top of the previous
  {\tt rsp} and move all register values to there. We need to copy them first because the newly created
  {\tt erim\_regs} maybe underneath our {\tt sigframe} so they are overlapped and get corrupted during moving.
  Then, we set the location of untrusted stack to this new {\tt erim\_regs} and return from the
  signal. This actually makes the signal delivering after {\tt sigreturn} easier because now {\tt sigreturn}
  will leave a legit {\tt erim\_regs} on the untrusted stack.

  Because when signal happens in untrusted domain, there will be a $128 bytes$ red-zone above
  the current {\tt rsp}. When allocating {\tt erim\_regs} on top of such stack, we must substrate
  {\tt rsp} for an extra $128 bytes$ so it will not interfere with red-zond, and
  at the end of {\tt syscall\_trap} we need to add the $128 bytes$ back to make the {\tt rsp}
  value correct. We replace the {\tt ret} instruction with {\tt ret \$0x80} for this.
  And, to ensure this is only one exiting point for {\tt syscall\_trap} and maintain,
  the consistence we add the extra $128 bytes$ in all cases including normal
  syscall invoking and direct signal delivering from signal handler.

  %So, we can first unwind the {\tt erim_regs} because they are useless now.

  \fi





==> figs/rnexpoline.tex <==

\begin{figure}

  \begin{tabular}{|c|}
    \hline \\
    \\
    \\
    \tikzmarkold[xshift=-\tabcolsep-2pt,yshift=-\RowDepth]{braceU} \hfill Address of Syscall \hfill \tikzmarkold[xshift=\tabcolsep,yshift=\RowDepth]{address} \\
    \hline  \\ \tikzmarkold[xshift=-\tabcolsep,yshift=-\RowDepth]{upperL}\hfill\hfill\tikzmarkold[xshift=\tabcolsep,yshift=-\RowDepth]{upperR} \\ \multicolumn{1}{c}{\tikzmarkold[xshift=-\tabcolsep,yshift=-\RowDepth]{bottomL}\hfill\hfill\tikzmarkold[xshift=\tabcolsep,yshift=-\RowDepth]{bottomR}} \\ \\  \\
    \hline \\ \\ 
    \hfill Syscall \hfill \tikzmarkold[xshift=\tabcolsep,yshift=\RowDepth]{syscall}
    \\
    Ret
    \\ 
    \hline \\ \\ \\ 
    \tikzmarkold[xshift=-\tabcolsep-2pt,yshift=-\RowDepth]{braceD} \hfill   \hfill 
    \\ 
    \hline
  \end{tabular}
  \begin{tikzpicture}[overlay,remember picture]
    \draw[snake=zigzag] (upperL) -- (upperR);
    \draw[snake=zigzag] (bottomL) -- (bottomR);
    \draw[->, bend left] (address) to (syscall);
    \draw[decorate,decoration={brace,amplitude=10pt,mirror}] (braceU) -- (braceD) node [midway, xshift=-1.2cm] {multiple pages};
  \end{tikzpicture}
  \caption{\textbf{Randmoized Trampoline}}
  \label{fig:trampoline}
\end{figure}


==> fork.tex <==
% --------------------
\subsubsection{\Code{Fork}}
%
\todo{remove me}
\label{sec:syscallvirt}
% --------------------

  % --------------------
  \arch calls for a user level only solution to prevent information flows that
  would expose protected segments.
  %
  In the operating system, as explored by Sirius~\cite{Tarkhani:EnclaveAware:2020}, this would mean
  integrating the \todo{...}.
  %
  \system makes this boundary explicit with the \sphere abstraction and as such
  we do \todo{...}.
  %
  \todo{think on what to write, i think it comes down to how we handle fork, but
    do we want to put that into the syscall section? Do we want to create a
  complete section on forking? Should this be that section?}



==> init.tex <==
  % --------------------
  \subsection{Initialization}
  % --------------------

  % --------------------
  \system loads the \td, allocates thread local data, including running status
  and separated stacks for the \td and \ud, registers a signal handler, and
  restricts \syscall privileges to \td \segments that are mapped to keys 0 and
  1.
  %
  %by using either a seccomp filter or Syscall User Dispatch~\cite{dispatch}.
  %
  %The filters ensure that \ud cannot invoke a system call.
  %
  %\todo{TODO: cite https://lwn.net/Articles/838502/}
  %
  %The \td \segments are mapped to keys 0 and 1 and the \ud \segments are mapped
  %to key 2.
  %
  %One challenge is assigning domains to MPK keys: Linux makes many assumptions
  %about always returning to key 0, which means the \visor must map itself into
  %that domain, however, it generates challenges because GLIBC assumes the
  %application runs with key 0. 
  %
  %We deliberately assign MPK key \Code{0} and \Code{1} for the \td.  The memory
  %pages with key \Code{0} will be accessible from both \td and \ud, but only
  %writable from \td while pages with \Code{1} are only accesible from \td.  
  %
  %This choice allows most kernel interactions with user to run with minimum
  %modification since it is the default key used by kernel, especially for
  %signal virtualization and CET, and key \Code{1} can be used for sensitive
  %data that must keep confidential (e.g. the location of syscall trampoline in
  %RIV nexpoline in section ??). \todo{FIXME: how should I refer RIV??  }
  %
  %After the initial steps, \system starts loading the initial executable binary
  %of the application. 
  %
  %The application is loaded with key \Code{2}, which we refer as \ud, if not
  %otherwise specified.
  %
  \system dynamically inspects the binary, remove \wrpkru from \ud code, and
  initializes \ud \segment permissions and maps with key 2.
  %
  The loader populates the stack with argv, envp, and auxv, and transfers
  control to the untrusted application by switching to the untrusted stack,
  reducing memory access permissions to the level authorized for the \ud, and
  jumping to the entry of the loaded executable. 
  %
  %At this point \system has successfully initialized its protection for
  %invariant~\ref{inv:memiso} and ~\ref{inv:sysexec}.
  %
  %In most time it would be a libc loader which serves as a secondary loader for
  %user application. 
  %
%  If the multi-domains are used to furture create subdomains in \ud, the libc
%  loader will load the corresponding libraries and invoke the subdomain
%  initializers in these libraries. After all subdomains settled down, the
%  \system will reject any request of creating either a sandbox or a safebox. 


==> model.tex <==
%%----------------------------------------------------------
\section{Intra-App Privilege Separation Model}
%
\label{sec:model}
%%----------------------------------------------------------

  In building on that, we observe that all prior generations neglected to
  observe system level flows from exposing protected segments.
  %
  Sirius~\cite{Tarkhani:EnclaveAware:2020} presents a similar solution but focuses on
  integrating the model into the kernel, which results in a complex
  implementation scattering checks and enforcement throughout the kernel
  requiring the kernel adhere to a novel intra-process abstraction.
  %
  Instead, we use the system call interface to check and enforce intra-app
  privilege separation within a single layer.
  %
  In this section we present the authority model for representing and protecting
  traditional memory based privilege separation.
  %
  Any privilege separation approach must consider protection from these
  resources as they offer critical ways to easily bypass existing models
  focusing narrowly on memory and control only.
  %
  This should serve as a starting point for any 4th generation privilege
  separation approach, and can be seen to be missing from all prior (save one)
  that would allow attacker easy access to protected segments.

  % --------------------
  Our goal is to avoid syscall filters with all-or-nothing course grained
  policies which lack programmability and compatibility for restricted domains.

  % --------------------
  \input{privmodel}

  % --------------------
  \input{sphere}

  % --------------------
  \input{sysflow}


==> old-sigvirt.tex <==

  % --------------------
  \subsection{Signal virtualization}
  %
  \label{sec:sigvirt}
  % --------------------
  \review{this was my hack job on the old one\ldots just
  added the above}.


    We must fully virtualize signals for two primary
    reasons.
    %
    First, signals expose processor state through
    \Code{struct sigframe}, potentially leaking sensitive
    state or allowing corruption of \pkru, which could lead
    to \ud control while in \td context (invariants
    I\ref{inv:sigintegrity} and I\ref{inv:memiso}).
    %
    %
    Third signals can interrupt \td execution, which could
    cause reentry into the \td, potentially corrupting
    internal state (violating atomicity invariant
    I\ref{inv:atomic} and protection invariant
    I\ref{inv:memiso}).
    
    \iffalse
    %
    Unfortunately, his is problematic because this will leak
    critical information from trusted domain to untrusted
    domain and ever worse, allowing them to modify certain
    registers and resume execution. They can also modify the
    PKRU register value in XSTATE which allows them to break
    MPK protection.  Also, untrusted application may not be
    able to handle signal correctly since the signal is from
    trusted domain. 
    %
    \fi

    % --------------------
    Full signal virtualization is challenging due to three
    reasons. 
    %
    First, Linux deterministically resets the \pkru state to
    a default value of being RW in \td and R for all others.
    %
    This means that regardless of whether the process was in
    \td or \ud mode, it returns in \td protection state.
    %
    Additionally, Linux pushes to the stack before switching
    the protection domain, which means that if the system
    was operating in \ud state prior to interrupt the signal
    stack must be in \ud or else the kernel will fault.
    %
    Second, signals interrupt asynchronously creating
    complex concurrency semantics for \system that must
    securely preserve standard signal semantics.
    %
    Third, \system must protect from reentry while
    maintaining those semantics.
    %
    Figure, 


    There are few other challenges of delivering signals to untrusted world caused by the kernel design. For exmaple, Linux kernel does not support specific 
    PKRU value when delivering signal. Instead, it is using a default PRKU value that allows reading and writing towards domain 0 while only allows 
    reading towards other domains. This will break our policy bacause even such semi-privileged status can be used to read trusted memory and elevate 
    from the `semi-trusted' domain to a real trusted domain while executing arbitrarily code. 

    As a result, we must create a signal virtualization layer that gives untrusted domain an illusion that all signals are delivered 
    while they are running and ensure that the code executing in trusted domain are totally transparent to untrusted domain. 
    We might in trusted domain at the time signal delivered by the kernel, but when we proxy the signal to untrusted domian, it will 
    see the registers values of the moment after trapped into our trusted domain. More specific, if they trapped because kernel interruped 
    in untrusted domain, we will simply passthrough the signal to the untrusted domian. Otherwise, we will deliver the signal when {\tt syscall\_trap}
    returns and set context accordingly to what untrusted domain should see after that return. 

    \subsubsection{Signal Trap Entrypoint}
    \label{sec:ste}
    Syscall virtualization allows us to intercept {\tt sigaction} syscall which registers a new signal handler in the kernel. 
    Instead of using the untrusted handler, we redirect the signal into our {\tt signal trap entrypoint} with flag = 
    {\tt SA\_ONSTACK} | {\tt SA\_SIGINFO} | {\tt SA\_RESTORER} | {\tt SA\_RESTART}. We also set the mask flag to mask all signals 
    so our entrypoint will never be re-entered by the kernel. 
    
    Here, {\tt SA\_ONSTACK} is a flag that set the signal stack to an alternative stack set by {\tt sigaltsatck}. This prevent signal to be delivered 
    directly into current stack which would make signal delivering harder. However, because kernel will use the immediate MPK to push sigframe into 
    the stack, we must put the stack into untrusted domain so kernel can always push into the stack no matter which domain we are currently in. 

    Any signal will then sent to this trusted handler, but in a `semi-trusted' domain. We have two things to do now, first we will utilize the `semi-trusted'
    domain to leave a proof that the signal frame is created by the kernel, after we switched to the trusted domain. This is because signal stack is in 
    untrusted domain, and this allows untrusted code to forge a sigframe in signal stack and jump into the entrypoint. 

    Since the only different between a signal sent by kernel or a signal forged by untrusted domain is that the kernel will switch into a `semi-trusted' domain,
    we must leave an evidence to the code after domain switching that we can read or write trusted data before we perform the switching. 
    After the switching, we will in trusted domain and we can verify the evidence to decide the next step. 

    The evidence we are using here is to write a `1' into a trusted memory. Because the entrypoint will not be re-entered, we can do this safely and 
    later after the switching, we can read the memory and check if there is a `1' and reset it to zero. The {\tt sig\_entry} is described in \ref{fig:entrypoint}.

    \begin{figure}
    \begin{lstlisting}[numbers=left]
sig_entry:
  movq $1, __flag_from_kernel(%rip)
  erim_switch
  cmpq $1, __flag_from_kernel(%rip)
  jne __sigexit
  movq $0, __flag_from_kernel(%rip)
  call _shim_sig_entry
    \end{lstlisting}
    \caption{\textbf{Signal Entrypoint}}
    \label{fig:entrypoint}
    
    \end{figure}

    After {\tt erim\_switch} we are in the trusted domain and {\tt \_\_flag\_from\_kernel} is in the trusted memory. If a untrusted code tried to jump into
    the signal entrypoint, there are few cases here. It can jump into the second line, but crash immediately because it trys to write a trusted memory without
    any privilege. Or it can jump to {\tt erim\_switch}, but the next {\tt cmpq} will find out the problem and reject the accessing. Jump to any lines after 
    {\tt erim\_switch} is meaningless because it will not grant them any privilege. 

    Re-entering of this function caused by first jump into it and then let a signal being delivered will not cause any problem because the untrusted code 
    cannot modify and trusted status and since kernel will not re-enter the entrypoint, the proofing operation for the real signal processing is atomic to 
    untrusted code: it will never see a  {\tt \_\_flag\_from\_kernel} equals to `1'.

    We will queue the signal after the switching, and depend on the originataion of the signal we will resume the execution of {\tt syscall\_trap} and delay 
    the signal or deliver a pending signal based on Linux's signal delivering rule immediately.

    \subsubsection{Signal Queue}

    \tikzset{
      queue/.style={
        rectangle, draw=black, thick, minimum width=1cm, minimum height=1cm
      }
    }

    \begin{figure}
      \begin{tikzpicture}
        \node[queue] (q64) {63};
        \node[queue, right= of q64] (q63) {62};
        \node[right=of q63] (qdot) {$\dots$};
        \node[queue, right=of qdot] (q2) {1};
        \node[queue, right=of q2] (q1) {0};
        \node[rectangle, draw=black, thick, minimum height=3cm, fit={(q64.west) (q1.east)}, inner sep=0pt, yshift=2.5cm] (kern) {Kernel};
        \node[rectangle, minimum height=1cm, fit={(q64.west) (q1.east)}, inner sep=-1pt, fill=gray!15, above=1 pt of kern.south, anchor=south] (kmask) {Signal Mask};
        \node[rectangle, draw=black, thick, minimum height=1cm, fit={(q64.west) (q1.east)}, inner sep=0pt, fill=gray!15, below=of qdot] (omask) {Override Mask};
      \end{tikzpicture}
      \caption{\textbf{Signal Queue;} Every signal queue can be masked seperately; When a signal is pending in our queue, the coressponding bit in kernel mask is set; Signal delivered from the smallest signal the largest; Kernel queue other pending signals for us. When override mask is set, signal deliver code will use that mask instead of the user set mask, the mask will then be reset. This allows some syscalls to be returned without delivering signal.}
      \label{fig:q}
    \end{figure}

    Inside intravirt, we managed a signal queue for each signal with a depth of 1. If the signal queue is fulled the coressponding signal will be masked immediately by setting
    masking bit in sigframe before returning from the entrypoint. This ensure that whenever a signal arrived, we can always handle it. 

    In the entrypoint, we first push the siginfo into the signal queue. Then, we check the origination of the signal. 
    If the signal comes from untrusted domain, we will choose one signal to be delivered into untrusted domain. Noticing that depends on the signal type and
    priority, we might choose to deliver another signal instead of current signal. That signal will be popped from the queue and we prepare the deliver 
    payload based on current sigframe and that signal info. 

    If, however, the signal comes from trusted domain, we will not deliver the signal until we are switching back to untrusted domain. In this case, we will 
    return back to trusted domain through {\tt sigreturn}.

    \begin{figure}
      \begin{tikzpicture}
        %\draw [help lines,use as bounding box] (-1,-4) grid (7,4);

        \fill[fill=purple!20] (-1.5, 2.5) arc[start angle=90,delta angle=-180,radius=2.5] -- cycle;

        \fill[fill=yellow!20] (5.5, 3.8) arc[start angle=0,delta angle=-180,radius=2.5] -- cycle;

        %\fill[fill=green!20] (7, 2) .. controls ++(205:1) and ++(-205:1) .. (4,0); %.. controls ++(-205:1) and ++(-230:1) .. (1,-1.5) .. controls (-230:1) .. (1, -4) -- (7,-4) -- cycle;
        \fill[fill=green!20] plot[smooth,tension=1] coordinates {(7, 1.5) (4,0.5) (1.5,-1.5) (1, -3.5)} -- (7,-3.5) -- cycle;

        \node[color=gray!45,scale=1.5,font=\bfseries\sffamily,rotate=90] (utt) at (-1,0) {Untrusted};

        \node[color=gray!45,scale=1.5,font=\bfseries\sffamily] (utt) at (3,3.5) {Semi-Trusted};

        \node[color=gray!45,scale=1.5,font=\bfseries\sffamily,rotate=-45] (utt) at (5,-1.5) {Trusted};

        \node[roundnodeL] (ut) at (0,0) {UT};
        \node[roundnodeL,align=center] (ssut) at (2,2.5) {Sig\\SmiUT};
        \node[roundnodeL,align=center] (sut) at (2,-2.5) {Sig\\UT};

        \node[roundnodeL,align=center] (sst) at (4,2.5) {Sig\\SmiT};
        \node[roundnodeL,align=center] (st) at (4,-2.5) {Sig\\T};

        \node[roundnodeL] (t) at (6,0) {T};

        \def\myshift#1{\raisebox{-2ex}}
        \draw[->, bend left,postaction={decorate,decoration={text along path,text align=center,text={|\sffamily\myshift|Syscall}}}] (ut) to (t);
        \def\myshift#1{\raisebox{1ex}}
        \draw[<-, bend right,postaction={decorate,decoration={text along path,text align=center,text={|\sffamily\myshift|Signal Deliver, Syscall Ret}}}] (ut) to (t);
        \draw[->, bend left,postaction={decorate,decoration={text along path,text align=center,text={|\sffamily\myshift|Recv Signal}}}] (ut) to (ssut);
        \draw[->] (ssut) -- (sut) node [midway] {Entrypoint};
        \def\myshift#1{\raisebox{-2ex}}
        \draw[<-, bend right,postaction={decorate,decoration={text along path,text align=center,text={|\sffamily\myshift|Direct Deliver}}}] (ut) to (sut);
        \def\myshift#1{\raisebox{1ex}}
        \draw[<-,bend left,postaction={decorate,decoration={text along path,text align=center,text={|\sffamily\myshift|Recv Signal}}}] (sst) to (t);
        \def\myshift#1{\raisebox{-2ex}}
        \draw[->,bend right,postaction={decorate,decoration={text along path,text align=center,text={|\sffamily\myshift|Defer Signal}}}] (st) to (t);

        \draw[->] (sst) -- (st) node [midway] {Entrypoint};

%        \node[fill=purple!20, 
      \end{tikzpicture}
      \caption{\textbf{State Transition with Signal;} UT:Untrusted; T: Trusted; Sig: Signal Handler, Signal masked by Kernel; Smi: Semi-Trusted Domain}
      \label{fig:state}
    \end{figure}

    \subsubsection{Signal delivering}
    \label{sec:signaldel}
    There are two cases for signal delivering, one is delivering a signal directly from the entrypoint and another is dieliver signal at the returning of 
    {\tt syscall\_trap}. 
    For any signal delivering routine, we will first allocate sigframe on untrusted stack (might be virtualized sigaltstack) as the kernel. Then, utilize the 
    return path (normal ret or sigreturn) as a trampoline to call the handler with the created sigframe. 

    In the entrypoint case, we read rsp of untrusted domain from signal and modify the rsp, rip, pkru, {\tt sig\_mask} and other gp registers in sigframe and return 
    from the signal, kernel will then help us to jump to the correct signal handler in userspace.

    In the syscall case, we read all registers for untrusted domain from a {\tt erim\_regs} we saved on the stack before we enter the syscall. 
    We put these value into sigframe and modify the rax to syscall return value and rsp before the {erim\_regs}. 
    Then, we modify the stack layout to allocate the sigframe and a new {\tt erim\_regs} frame. The new {\tt erim\_regs} contains the registers value
    for the signal handler in untrsuted domain as the sigframe we used in previous case.
    After we return,
    erim will pop the {\tt erim\_regs} all registers as an normal returning from syscall. But instead of returning to where the {\tt syscall\_trap} was called, 
    it returns to the untrusted signal handler and starts to handle the signal. One difference here is we need to manually set signal mask to unmask the 
    delivered signal after we finish using the siginfo data to allow next signal comes from kernel. 
    
    \begin{figure*}[h]
      %\subfloat[Stack layout when delivering signal directly from Signal Entrypoint]{
        \begin{subfigure}[t]{.45\textwidth}
        {
        \begin{tabular}{|c|c|c|}
          &  &       \\ \cline{3-3} 
                              &  &   \tikzmarkold[]{news1} trampoline address    \\ \cline{3-3} 
                              &  &  Signal Frame  \\ 
                              &  &    Signal Info \\ \cline{1-1} 
          trampoline address  &  &\tikzmarkold[]{rsp2l}\hfill rsp \hfill\tikzmarkold[yshift=0.33ex]{rsp2r}\\  \cline{1-1}
          Signal Frame        &  &\tikzmarkold[]{rip2l}\hfill rip \hfill\tikzmarkold[]{rip2r}\\
          Signal Info         &  &    other regs  \\
\tikzmarkold[]{rsp1l}\hfill rsp\hfill\tikzmarkold[]{rsp1}&  &                \\
\tikzmarkold[]{rip1l}\hfill rip\hfill\tikzmarkold[]{rip1r}&  &    XSTATE      \\
       other regs             &  &                \\ 
                              &  &                \\ \cline{3-3}
           XSTATE             &  &   \multirow{2}{*}{Red Zone}     \\
                              &  &                \\  \cline{3-3}
                              &  &\tikzmarkold[]{orgs1l}\hfill Original Stack\hfill\tikzmarkold[]{orgs1r} \\ \cline{1-1} \cline{3-3}
          \multicolumn{1}{c}{Signal Stack}        & \multicolumn{1}{c}{}  & \multicolumn{1}{c}{User Stack} \\
          \multicolumn{3}{c}{} \\
          \multicolumn{3}{c}{} \\
        \end{tabular}
        }
        \begin{tikzpicture}[overlay, remember picture]
          \draw [->] (rip1r) .. controls ++(0:8mm) and ++(180:8mm) .. (rip2l);
          \draw [->] (rsp1) .. controls ++(0:8mm) and ++(180:8mm) .. (news1);
          \draw [<-] (rsp1) .. controls ++(0:8mm) and ++(180:8mm) .. (orgs1l);
          \draw [->, bend left] (rsp2r) to (orgs1r);
        \end{tikzpicture}
        \caption{Stack layout when delivering signal directly from Signal Entrypoint}
      %}
      \end{subfigure}
      \hfill
      %\subfloat[Stack layout when delivering signal after syscall]{
        \begin{subfigure}[t]{.45\textwidth}
        \begin{tikzpicture}[overlay, remember picture]
          \coordinate (regsLLL) at  ([yshift=1.5mm]pic cs:regsLL);
        \node[rectangle, fit={(regsLLL) (pic cs:regsRR) (pic cs:regsLR)}, draw=black, thick, fill=gray!10] (regbox) {};
        \end{tikzpicture}
        {
        \begin{tabular}{|c|c|c|}
          &  & \hfill\hfill \tikzmarkold[xshift=\tabcolsep,yshift=-\RowDepth]{nrsp1} \\ \cline{3-3} 
          &  & \multirow{2}{*}{erim regs} \\ 
          &  &                            \\ \cline{3-3} 
          &  & rip=handler                     \\ \cline{3-3} 
          &  & trampoline address         \\ \cline{3-3} 
          &  & Signal Frame               \\
          &  & Signal Info                \\
          &  & \tikzmarkold[]{newrsp}\hfill rsp\hfill\tikzmarkold[xshift=\tabcolsep,yshift=\RowDepthT]{newrspR}\\
          &  & \tikzmark{regsLL}rip                        \\
          &  & \tikzmark{regsLR} other regs \tikzmark{regsRR}                \\
          \tikzmarkold[xshift=-\tabcolsep,yshift=-\RowDepth]{orsp1} \hfill\hfill &  &                            \\ \cline{1-1} 
          \hfill\multirow{2}{*}{erim\_regs}\hfill\tikzmarkold[xshift=\tabcolsep,yshift=-\RowDepth]{eregs} &  & XSTATE                     \\ 
                    &  &                            \\\cline{1-1} 
          \hfill rip\hfill\tikzmarkold[xshift=\tabcolsep,yshift=-\RowDepth]{retspo}  &  &  \hfill\hfill\tikzmarkold[xshift=\tabcolsep,yshift=-\RowDepth]{retsp}  \\ \cline{1-1} \cline{3-3} 
          \multicolumn{1}{c}{User Stack Before}           & \multicolumn{1}{c}{} & \multicolumn{1}{c}{User Stack After}           \\
          \multicolumn{1}{c}{}         &\multicolumn{1}{c}{}  &  \multicolumn{1}{c}{}                          \\ \cline{1-1} \cline{3-3} 
          \tikzmarkold[xshift=-\tabcolsep,yshift=\RowDepthT]{osp2}User Stack Pointer         &  & User Stack Pointer   \tikzmarkold[xshift=\tabcolsep,yshift=\RowDepthT]{nsp2}      \\ \cline{1-1} \cline{3-3} 
          \end{tabular}
        }
          \begin{tikzpicture}[overlay, remember picture]
            \draw[->, bend left] (osp2) to (orsp1);
            \draw[->, bend right] (nsp2) to (nrsp1);
            \draw[->] (eregs) .. controls ++(0:8mm) and ++(180:8mm) .. (regbox.west);
            \draw[->, bend left] (newrspR) to (retsp);
          \end{tikzpicture}
          \caption{Stack layout when delivering signal after syscall}
      %}%
      \end{subfigure}
      \caption{Stack Layout for Signal Delivering}
    \end{figure*}

    \subsubsection{Signal Return}

    We will put the trampoline for returning from the signal just like the kernel. However, we will call a {\tt syscall\_trap} to our virtualized {\tt sigreturn} instead of using syscall instruction.

    There are few things in the signal frame we need to sanitizer. We need to set the queue mask by the masking in sigframe and modify the signal's masking to the real mask we need 
    for the kernel. Another thing is {\tt stack\_t} used by {\tt sigaltstack}, we set our virtualized {\tt stack\_t} and reset this to the signal stack for 
    our entrypoint.
    We also need to ensure the PKRU in XSTATE has beed set to untrusted domain. 

    After checking all the arguments, we set our {\tt rsp} to the sigframe and jump directly to our syscall trampoline. 
    The kernel will assist us to switch back to untrusted domain using the value in sigframe.

    One special case for signal return is that we need to deliver a signal immediately after signal return. 
    In order to deliver the signal, we can not use {\tt sigreturn} syscall to jump into previous context. 
    This is also not the normal deliver signal after syscall scenario because sigreturn actually failed 
    in this case. Out currently choice here is to move the {\tt rip} in {\tt erim\_regs} 6 bytes before current 
    position and {\tt rax} to {\tt NR\_rt\_sigreturn} to restart current syscall.
    Now, although the syscall failed, in the next time we returned from the new signal, we 
    will recall sigreturn syscall again to sigreturn from previous siganl again. 

  


==> osdi.arch.tex <==
%%----------------------------------------------------------
\section{Nested Separation Architecture}
%
\label{sec:osdiarch}
%%----------------------------------------------------------
  
  % --------------------
  \system is a userlevel intra-privilege separation framework, but unlike prior
  efforts it emphasizes full virtualization of system calls and signals, as well
  as exposes several complex artifacts that were neglected by prior work.
  %
  Our challenge is to insert the security monitor into the application's runtime
  and ensure all \syscall uses go through \system and signals are properly
  virtualized without being slower than ptrace or bypassable.
  %
  By doing this, \system is able to assert any policy and emulate access to
  system resources while ensuring monitor isolation.
  %
  In this section we provide an overview of the approach, define the properties
  and policies required for a privilege separated nested execution environment,
  and describe the design philosophy.
  
  % --------------------
  \input{principles} 

  % --------------------
  \input{overview}
  
  % --------------------
  \input{org} 
  
  % --------------------
  \input{properties}
  
  % --------------------
  \input{boxing}

  \iffalse

  %%--------------------------------------------------------
  \subsection{Overview}
  %
  \label{sec:principles}
  %%--------------------------------------------------------

    % --------------------
    Intra-process privilege separation is like creating a
    virtual privilege ring 

    how dif than sfi?

    % --------------------
    The goal of \arch is to virtualize access to the set of
    resources available within a process, which includes
    both CPU and memory state.
    %
    Various techniques exist for both, from managed language
    runtimes to memory virtualization like SFI etc.
  

  \fi
  
\iffalse
- An efficient and simple (new sec model into kernel
    complex) way to realize \model
    - Any single address space approach has to have the
      boxes/components that are described here
  - Creating the equivalent to a virtual privilege switch,
    ie priv level with all mechanism
      - THis is why nexpoline is like a syscall, secure
        transition into priv mode
\fi

\iffalse
  
  % --------------------
  The value of specifying the \model model at the \syscall layer is that it can
  be enforced either inside or on top of the OS.
  %
  Since performance is an essential element of fine-grained privilege
  separation, intra-process separation architectures are essential.
  %
  However, besides lacking \model policies they neglect several key aspects of
  low-level control and data flow integrity, which can undermine the system.
  %
  In this section, we take a bottom up approach to describing a nested
  separation architecture that extends the \domain abstraction with key objects
  required to protect.
  %
  The key result is the definition of a standard interface and required
  properties and invariants that any nested separation kernel must provide for
  safe execution.

  % --------------------
  Security monitors are responsible for asserting protection properties, and
  have been done by many layers and implementations.
  %
  Some have become somewhat generic terms---hypervisor, microvisor, microkernel.
  %
  In this section we detail a architecture aimed at providing a similar
  \emph{visor} like definition specifically for flat address space,
  intra-separation, heterogenous resource types. 
  %
  The key emphasis for this distinct from our prototype is that we believe there
  are several ways to insert monitoring over system calls, virtualize signals,
  and assert the \model policies, and believe this general description provides
  the proper encapsulation boundary while making several parts of program and
  processor state first class objects demanding protection.
  %
  How to protect these are left to a particular instance of the architecture.

  % --------------------
  The primary characteristic the \arch is to nest the monitor at a single
  privilege level and in the same address space of the privilege separated
  process, thus enabling enable lightweight and efficient protection.
  %
  Much like single-address space systems of the past~\cite{Mondrix, etc., SFI},
  we specify both an abstract protection system interface and protection model,
  as well as systematically express essential properties and policies for such a
  solution. 
  %
  %We also systematically express essential properties and policies for such a
  %solution, paying careful attention to the unique security constraints. 
  %
  In this section, we take a top down approach, first detailing our design
  philosophy, then providing an overview, and concluding with a series of
  detailed properties that any nested userlevel monitor must adhere to.
  %
  The \arch architecture described here details a general organization, which
  can be implemeted with many mechanisms---popular approaches include nested
  page tables, secure execution environments, software fault isolation, or
  protection keys. 
  %
  We describe a protection key instance of the \arch in the next section.

  % --------------------
  We specifically instantiate our priv model as intra-priv sep because of
  performance and more importantly the complexity of the kernel, yes there are
  tradeoffs but we want to know how far this direction can go.


  % --------------------
  \arch is a userlevel intra-process privilege separation architecture, but
  unlike prior efforts, \arch provides a more complete set of objects to protect
  along with support for facilitating client applications.
  %
  Our challenge is to insert the security monitor into the application's runtime
  and represent all system objects to deny malicious information flows without
  being slower than ptrace, which simulates state of the art multi-process
  privilege separation approaches.
  %
  Not only does \arch prevent attacks on the monitor isolation itself, it can
  also enable a unique class of efficient multi-principle, sub-process system
  object policies.
  %
  The goal of this section is to present a low-level virtual machine like
  interface for the set of capabilities and basic organization of such a
  protection system, and to explore a unique set of mechanisms for realizing the
  architecture in \S~\ref{sec:design}.
  %
  The key elements of \arch include: 1) a privilege model, 2) an architecture
  definition and associated policies, and 3) an interface for facilitating app
  compartmentalization.
  
  \fi

  \iffalse

  \todo{I've dumped stuff here}

  % --------------------
  WE extend the def of the protection context because we have other first class
  primitives that need protected: instructions and cpu registers.
  %
  A key object missed by existing work is information that is in the CPU, which
  requires proper virtualization to ensure isolation.
  %
  As such we include instruction capabilities into our model, that is a list of
  valid instructions a given domain is authorized to invoke, which is an
  essential ingredient to MPK based approach and exposes subtle but critical
  information flows that allow attackers to bypass state of the art systems. 

  %
  In this model\ndd{maybe sentence is moved to later... yes we don't talk about
  switches here at all}, a domain is permitted to transfer control (\eg
  \Code{jmp}) to any in-memory segment address, however, without a context
  switch the system will not transition the \domain and thus no new access will
  be obtained (a privilege escalation attack)\footnote{This design choice could
  allow side-channels to persist and must be revisited in future work when
adding it into the threat model.}

  % --------------------
  When doing a context switch it's too costly to swap out and make NX, so we
  ellude that which creates problems...

  \fi
  


==> overview.tex <==
%\subsection{Overview and Properties}

\iffalse
% --------------------
  \begin{figure*}[]
      %
      \begin{center}
        \includegraphics[width=\textwidth]{figs/arch}
      \end{center}
      %
      \caption{\label{fig:sysarch}
        %
        \system Architecture.
        %
      }
  %
  \end{figure*}

\fi

 % \input{priv-tbl}
  % --------------------
  \system is a 4th generation approach that fully virtualizes privilege and
  prevents bypass attacks.
  %
  \system injects the monitor into the application, as the \td, and removes the
  ability of the \ud to directly modify \emph{privileged state}.
  %
  Privileged state includes: protection information (\pkru and memory mappings),
  code, \monitor code and data, direct system call invocation, raw signal
  handler data, CPU registers on transitions and control-flow.
  %
  The \monitor is inserted on startup by hooking all system call execution and
  initializing the protection state so that the \td is isolated with no files
  opened or mapped.
  %
  %There are three major subsystems in \system that are each dependent on the
  %others to maintain isolation: privilege (memory), syscall, and signal
  %virtualization.
  % --------------------
  %\paragraph{Invariants}

  % --------------------
  \todo{These are old and need updated. Remove this comment once we have a
  draft} To summarize the design we present the following properties/invariants
  which are the topic of the rest of the section:
    %
    %To derive this set of invariants we combine PKU Pitfalls as well as our own
    %invariants.
    %
    %The high level property can only be achieved when the following are
    %
    \begin{inv} Direct Access Integrity:
      %
      \label{inv:memiso}
    %
    \ud never executes while \pkru is in \td in context.
    %
    \end{inv}
    %
    \begin{inv} Code Execution Integrity:
      %
      \label{inv:codeexec}
    %
    All \ud code is validated prior to being mapped $W \oplus X$.
    %
    \end{inv}
    %
    %\begin{inv} Guaranteed Mediation or Protected Call Gates:\end{inv}
    %
    \begin{inv} Syscall Execution Integrity:
      %
      \label{inv:sysexec}
    %
    Prevent \ud from directly executing \syscall.
    %
    \end{inv}
    %
    %\begin{inv} Indirect Access Integrity:
    %%
    %As previously indicated, \syscalls allow memory access through many kernel
    %interfaces, all need to be denied.
    %
    \begin{inv} Protection Context Integrity:
      %
      \label{inv:mapping}
    %
    Trusted domain memory never mapped into the \ud context.
    %
    \end{inv}
    %
    \begin{inv} \syscall Access Integrity:
      %
      \label{inv:iaccess}
    %
    Access through sudo filesystems (procfs) is denied.
    %
    \end{inv}
    %
    \begin{inv} Atomicity of Monitor:
      %
      \label{inv:atomic}
    %
    Trusted domain operates atomically from the perspective of the \ud.
    %
    \end{inv}
    %
    %% Like this but didn't fit yet
    %%\begin{inv} Monitor Exit Integrity:
    %%
    %Control never leaves the monitor without going through exit gate, which is
    %essential as signal virtualization
    %%adds an interface to spoof signals which can influence
    %%control in the monitor.
    %%
    %\end{inv}
    %
    \begin{inv} Signal Handler Integrity:
      %
      \label{inv:sigintegrity}
    %
    Signal handler context is not directly corruptible by \ud.
    %
    \end{inv}

  % --------------------
  Invariants \review{x} and \review{y} are enforced by single privilege level
  memory isolation using MPK.
  %
  \todo{Write a short description of memory isolation, \wrpkru caps, ref erim}. 


  % --------------------
  The other invariants are the topic of original investigation in this work and
  are described in the remainder of the section.


  \iffalse

  % --------------------
  \paragraph{Privilege and Memory Separation}
  partitions the application into two spaces, \td and \ud,
  and uses \wrpkru to switch between the two domains, which
  changes the accessible set of memory.
  %
  Access to \wrpkru instructions for malicious uses is
  prevented by using a technique we call \emph{instruction
  capabilities}.
  %
  The primary requirement of privilege virtualization is to
  \emph{ensure the \ud does not gain control of execution
  while in the \td mode.}
  %\begin{prop} ensure monitor state remains isolated (not
  %accessible or corruptible) from the \ud.  \end{prop}

  % --------------------
  \paragraph{System Call Virtualization} ensures that all
  \syscalls are only executed by \td and additionally
  supports any combination of none, partial, and unmodified
  \syscall support by using instruction capabilities.
  %is provided by a technique forcing all \syscall
  %operations through the monitor, again using instruction
  %capapbilities to ensure the \ud cannot invoke one
  %directly.
  %
  %System call virtualization asserts two key requirements:
  %
  %\begin{prop} only the monitor can invoke \syscall
  %instructions \end{prop}
  %%
  %\begin{prop} prevent monitor isolation bypass through
  %system interfaces \end{prop}
  %%
  The challenge is stopping the \ud from
  generating/injecting its own syscall instruction or
  finding unintended ones. CPI blocks access to unintended
  syscall instructions but that would add a substantial performance
  cost to the system.
  %
  Instruction capabilities operate similarly protection
  rings where the \ud is denied use of the instructions using
  any combination of language based security mechanisms.
  %
  \system uses its control over \syscalls to ensure that \td
  memory is never made accessible to the \ud through system call
  resources.
  %

  % --------------------
  \paragraph{Signal virtualization} is achieved by setting
  up a virtual signal queue in \system that effectively
  replicates what the kernel is doing.
  %
  Securely managing signals turns out to be one of the
  biggest challenges because the virtualization technique
  opens up a small interface that could be used to attack
  \system as well as demands complex concurrency control.
  %
  Signal virtualization ensures that raw signal handler
  and CPU state are not accessible to the \ud, which could be
  corrupted to manipulate memory protection policies or
  control-flow of \td, and that all signals are handled
  atomically to avoid corruption of \system runtime.
  %
  %\begin{prop}
  %%
  %1) prevent corruption of privilege CPU state accessible
  %to handlers (\ie \pkru value),
  %%
  %\end{prop}
  %%
  %\begin{prop}
  %%
  %2) prevent atomicity violations that would lead to \ud
  %gaining control while in \td context, and
  %%
  %\end{prop}
  %%
  %\begin{prop} 3) intercept faked signals that are a
  %byproduct of virtualizing signals in usermode.
  %%
  %\end{prop}

\fi


\iffalse
  % --------------------
  The fundamental goal of \system is to preserve the
  integrity of the nested security monitor within
  intra-separation systems.
  %
  This is a different objective than the protection systems
  themselves, which have diverse abstractions from exclusive
  access to sandboxing.
  %
  We then specialize a set of security properties that must
  be in place given the specific mechanisms we've chosen and
  perform a systematic analysis of all system calls to
  identify sensitive and non-sensitive operations.
  %
  After that we define a set of policies that must be
  enforced in order to uphold the high level security
  property.
  %
  The overall theme of the description in this section is to
  specify a base configuration of the system which adheres
  to an initially secure system and then to identify the set
  of transition relations that can change the configuration,
  and to establish rules for each transition so that the
  system will always maintain a safe state.

\fi


  \iffalse
  % --------------------
  Our approach is to combine prior work on nested execution
  monitor isolation with new techniques to eliminate threats
  from signals and system calls.
  %
  The result is a new privilege separation framework that
  virtualizes all system calls and signals by inserting a
  monitor and emulating.
  %
  By doing this \system is able to assert any policy it
  desires, \eg deny all, allow subset, allow but deny some
  functionality.
  %
  As indicated, ptrace could do this but would result in a
  prohibitively slower mechanism.
  %
  Instead, we nest the monitor within the process
  itself and provide a set of properties with four
  separate mechanisms as depicted in
  Figure~\ref{fig:sysarch}.
  % --------------------
  \fi




==> priv-tbl.tex <==
\begin{tabular}{ | l | c | r | l | }
  \textbf{Operation} & \textbf{Access Method} & \textbf{Policy} & \textbf{Mechanism} \\\hline
\end{tabular}


==> privsep-bg.tex <==
  %%--------------------------------------------------------
  \subsection{Privilege Separation}
  %%--------------------------------------------------------
    % Point: Define basic terminology and protection model, why? So that in the
    % app/des I can directly say what we are isolating without needing to tie it
    % to some abstraction model.
    % --------------------
    In \emph{privilege separation} an application is partitioned so that the
    various parts cannot access other parts.
    % Anjo: why use parts here instead of component as used above?
    %
    The protection system enforces policies by separating the application into
    distinct \emph{domains} and protecting each domain's \emph{objects}.
    %
    \emph{Privilege} is typically defined as either \emph{execution-of} or
    \emph{access-to} other component code and data.
    %
    %Protection can be enforced with any number of mechanisms, and the policy
    %can vary widely.
    %
    There are a few high level models: sandboxing, safeboxing, or
    compartmentalizing.
    %
    In sandboxing, buggy or untrustworthy code is restricted from accessing most
    resources~\cite{Yee:Native:2009}.
    %
    In contrast, a safebox restricts access of a subset of state to a small
    trusted component~\cite{Provos:Preventing:2003}, \ie protected
    subsystems~\cite{Lampson:Protection:1974, Saltzer:Protection:1975}.
    %of Saltzer and Schroeder~\cite{Saltzer:Protection:1975}.
    %
    %---the original work by bla and bla~\cite{} introduced this model which has
    %become standard, but it is no different from any high and low privilege
    %split system, \eg supervisor vs usermode.
    %
    Compartmentalizing, decomposes an application into multiple mutually
    distrusting components, which requires abstractions for isolation and
    sharing~\cite{Brumley:Privtrans:2004, Bittau:Wedge:2008,
    Vasilakis:Automated:2018}.
    %
    %The key point is that all use a base privilege split: a separation
    %kernel~\cite{Rushby:Design:1981} isolates and controls sharing and
    %communication.
    % -------------------- POINT: specify the property that we can show breaks
    % So we want to define the highlevel prop so we can see how low-level flows
    % trivially bypass
    % --------------------
    The core abstraction of privilege separation is the protected memory
    segment, \ie to treat each segment of virtual memory as a first class object
    and manage data access to it.
    %
    The elemental properties are 1) memory segments only accessed from permitted
    code, 2) controlled entry and exit to subsystem (where memory segment
    switching ocurss), and 3) controlled data sharing or message passing.


==> properties.tex <==
  % --------------------
  \paragraph{Nested Monitor Property}
  %
  \label{sec:nestedprop}
  % --------------------

    % --------------------
    We provide the following informal description of a high
    level property and a set of invariants that ensure the
    property.
    %
    The basic property is that:
    %
    \begin{prop}
    %
    Privilege Separation Integrity: All privileged bits,
    whether CPU register state or memory, cannot be modified
    or accessed by the \ud.
    %
    \end{prop}
    %
    Care must be taken when attempting to break down the
    properties because the nested model makes certain state
    accessible---in contrast to traditional ring-based
    protection models.
    %
    In a sense, these properties ensure a virtual protection
    ring within the process and address space.
    %
    Our method for describing correctness is inductive: the
    system starts in a state where the \td and \ud are separated
    and all protection bits are in place.
    %
  \iffalse
  %
  The basic properties enforced:
  %
  \begin{prop} Nested Monitor Integrity\end{prop}
  %
  \begin{prop} Syscall Virtualization\end{prop}
  %
  \begin{prop} Signal Virtualization\end{prop}
  %
  Direct monitor integrity is enforced using MPK based
  isolation (as explored by ERIM/Hodor/etc).
  %
  Due to the complexity of the system interface, the
  monitors isolation depends on both system call and signal
  virtualization.
  %
  Syscall virtualization is achieved through a monitor that
  removes the ability of the \ud to execute a system call
  directly, forcing all calls through the monitor.
  %
  Specifically, we introduce a new mechanism that uses
  seccomp to restrict system call execution to a small
  region of memory and then use randomization to locate the
  instruction.
  %
  %\system forces system call control by using a simple
  %seccomp filter, however, because \system is nested in the
  %address space and we must be able to execute \syscall
  %without first transitioning to the kernel, we need to
  %leave it mapped into the address space.
  %%
  %This means that its location could be identified and then
  %directly executed by the \ud.
  %%
  %Thus we must ensure that such a control flow cannot
  %happen, which we solve with a new lightweight instruction
  %randomization technique.
  %
  Signals can expose low-level protection state (\pkru) and
  also generate subtle control flow behavior that if left
  unchecked could allow the \ud to gain control while memory
  permissions are set for the \td.
  %

  \fi


\iffalse
  %
  System asserts isolation by ensuring each modification or
  transition to protected operations does not invalidate the
  following properties:
  %
  \begin{prop} Monitor Access Integrity:\end{prop} while the \ud
  is executing all monitor state is protected from read and
  writes.
  %
  %\begin{prop} Guaranteed Mediation or Protected Call
  %Gates:\end{prop}
  %
  \begin{prop} Monitor Control Integrity: privilege state
    can only be modified if the monitor is entered through a
    protected call gate, ensuring that all protection
    policies are asserted.  \end{prop}
  %
  \begin{prop}Syscall Execution Integrity:
  %
  prevent \ud from directly executing \syscall. The
  challenge is stopping the \ud from generating/injecting
  it's own syscall instruction or finding unaligned ones.
  Could solve this with CPI but that would add an automatic
  high performance cost to the system. Can we do it more
  economically?
  %
  \end{prop}
  %
  \begin{prop} System Bypass Integrity:\end{prop}
  %
  \begin{prop} Signal Virtualization and
    Integrity:\end{prop}
  %
  \begin{prop} Direct Memory Protection:\end{prop}
  %
  \begin{prop} Atomic Monitor:\end{prop}
  %
  \begin{prop} Monitor Exit Integrity:\end{prop}  Control
  never leaves the monitor without going through exit gate:

  % --------------------
  \system forces control using a simple seccomp filter,
  however, because \system is nested in the address space
  and we must be able to execute \syscall without first
  transitioning to the kernel, we need to leave it mapped
  into the address space.
  %
  This means that its location could be identified and then
  directly executed by the \ud.
  %
  Thus we must ensure that such a control flow cannot
  happen, which we solve with a new lightweight instruction
  randomization technique.
  %
  \system ensures that it's runtime is protected from
  compromise by using MPK based single-privilege level
  virtualization as introduced by ERIM.
  % --------------------
  %Nesting and virtualizing privilege creates unique
  %challenges for system call virtualization, the obvious
  %being to 1) ensure system calls only originate from the
  %\td and  2) \td state is protected.
  %%
  %Less obviously, \system must isolate the monitor from
  %access through system objects and signal abuse, both of
  %which can influence data layout, access control policies
  %for memory regions, and control flow.
  %
  As indicated, protection of the monitor also depends on
  proper isolation from indirect attack through system calls
  and signals.
  %
  Signals turn out to add the most complexity as
  virtualizing them create unique corner cases that an
  attacker might be able to abuse.
  %
  %To isolate the monitor, we must protect against three
  %main classes of attack: 1) direct memory and control-flow
  %protection, 2) memory access through system calls, and 3)
  %memory and non-control data attacks through signal
  %manipulation.

  \fi

  % --------------------
  %\subsection{Privileges}
  % --------------------
  %The privileges in our system include access to: syscall
  %instruction, PKRU regs, alias control, etc.


  % --------------------
  %\subsection{Privileges: Objects to Protect}
  % --------------------
  %  Privileges: What are we protecting and why?

  % --------------------
  %\subsection{Attacks}
  % --------------------
  %- Attacks: How to compromise and classification?

  % --------------------
  %\subsection{New Attack Vectors}
  % --------------------
  %- Syscall Attack Vectors
  %- Signal Attack Vectors

%%%%% TODO
\iffalse %TODO flessh it out
    % --------------------
    Unfortunately, despite the sophisticated and working
    machinery, Linux/POSIX provides interfaces through
    kernel objects that allow the basic property to be
    bypassed.
    %
    PKRU Pitfalls paper did some analysis to expose this
    class of threats and we briefly summarize here, as they
    lay the foundation to \system design as well as a few
    new attacks we expose in this work.

    \writeme{Fill this out in five ish subsections}

    %%--------------------------------------------------------
    \paragraph{}
    % --------------------

\fi

\iffalse
  % --------------------
  \subsection{Security Policies}
  % --------------------

    % --------------------
    \paragraph{Alias Integrity}
    %
    As prior work on intra-privilege virtualization noted, a
    key aspect of protection for intra-level separation is
    that protection is typically enforced on the mappings
    between virtual and physical resources.
    %
    The whole idea of virtualization is built on this fact,
    therefore, any policy or alias that might insert a new
    unmediated access edge must be protected against.
    %
    Of course building security into (modify Linux like
    lwcs) or below the OS (virtualization hardware, or like
    more recent Donky hardware that enables user level
    monitor isolation), however, the high level property
    remains the same.

    % --------------------
    \paragraph{Mapping Policies}
    %

    % --------------------
    \paragraph{\syscall Instruction Capabilities}
    %
    Unlike the \wrpkru instruction that is long enough to be
    removable from the runtime, \syscall is a \review{2}
    byte sequence and not as easily removed, given many
    false positives.
    %
    As such we needed to devise an alternative method for
    ensure this property.

    % --------------------
    \paragraph{Signal Protections}
    %

    \fi


==> rw-tbl.tex <==
  % --------------------
  \begin{table}[t]
    {{\scriptsize
      %
      \def\arraystretch{1.0} % changes vertical space scale
    %
    \newcommand*\no[1][0.6ex]{\tikz\draw (0,0) circle (#1);} 
    \newcommand*\halfy[1][0.6ex]{%
      \begin{tikzpicture}
      \draw[fill] (0,0)-- (90:#1) arc (90:270:#1) -- cycle ;
      \draw (0,0) circle (#1);
      \end{tikzpicture}}
    \newcommand*\yes[1][0.6ex]{\tikz\fill (0,0) circle (#1);} 
    \begin{tabularx}{\textwidth}{l X X X X X X X X}
      % System | Feature 1 | f2 | ... 
      %
      \textbf{System}   & \rotatebox{25}{\textbf{Data Flow}} &
      \rotatebox{25}{\textbf{Control Flow}} & \rotatebox{25}{\textbf{System
      Flow}} & \rotatebox{25}{\textbf{\syscall Monitor}} &
      \rotatebox{25}{\textbf{Signal}} & \rotatebox{25}{\textbf{Multi-Process}} &
      \rotatebox{25}{\textbf{Concurrency}} & \rotatebox{25}{\textbf{Multi-Domain}} \\
      %
      %\textbf{System}   & \rotatebox{25}{\textbf{Data Flow}} & \rotatebox{25}{\textbf{Control Flow}} & \textbf{SF} & \textbf{SM} & \textbf{Sig} & \textbf{MP} & \textbf{MT} & \textbf{MD} \\
      %
      \toprule
      %
      %System       (direct) Data Flow     ControlF   Sys     Monitor    Sig         MultiProc       MultiThread   MultiDomain
%      LwC         & \checkmark & \checkmark & $\times$ & $\times$ & $\times$ & $\checkmark$ & $\checkmark$ & $\checkmark$\\
      %
%      Wedge/Dune         & \checkmark & \checkmark & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$\\
      %
      Erim~\cite{Vahldiek-Oberwagner:ERIM:2019}/Hodor~\cite{Hedayati:Hodor:2019}        & \yes & \halfy & \no & \no & \no & \halfy & \halfy & \no\\
      %
      %John Alt          & \checkmark & \checkmark & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$\\
      %
      SMV~\cite{Hsu:Enforcing:2016}               & \yes & \yes & \halfy & \halfy & -- & \yes & \yes & \yes\\% 
      %
      Shreds~\cite{Chen:Shreds:2016}            & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes\\
      %
      SeCage~\cite{Liu:Thwarting:2015}            & \yes & \yes & \yes & \halfy & \yes & \yes & \yes & \no\\
      %
      Enclosure~\cite{Enclosure}        & \yes & \halfy & \halfy & \no & -- & \halfy & \halfy & \yes\\
      %
      Sirius~\cite{Tarkhani:EnclaveAware:2020}*           & \yes & \yes & -- & -- & -- & -- & -- & -- \\
      %
      \system           & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes \\
      %
      \bottomrule
      %
    \end{tabularx}
    
    \caption{\label{tbl:barf} Comparison of low-level isolation properties and
    features of native code intra-process mechanisms. 
    %
    %DF = Data Flow. CF = Control Flow. SF = System Flow. SM = Syscall monitor. Sig = Signal control and data flow. MTI = Multithreaded memory isolation. MP = Data flow across address space in fork process model. MT = Multithreaded safety concurrency.  MD = Multidomain control and data flow security. 
    %
    This table presents a minor contribution of the work as it presents a more
    complete and holistic taxonomy of features IPI must consider in a 4th
    generation approach. *Sirius uses a different mechanism (SGX) and threat
    model. \review{rows/cols unfinished!!!!}
    %
    }
    %
    }}
    %
  \end{table}
  


==> seceval.tex <==
%%----------------------------------------------------------
\section{Security Evaluation and Analysis}
%
\label{sec:seceval}
%%----------------------------------------------------------

% --------------------
Here we detail how we ensure our system is secure.
%
The basic idea is to qualitatively reason about threat
vectors and to implement several attacks and ensure the
protection system denies access.
%
\writeme{fangfei write me\ldots}

% --------------------
\subsection{Memory Protections}
%
\label{sec:secevalmem}
% --------------------

% --------------------
\subsection{\syscall Bypass}
%
\label{sec:secevalscall}
% --------------------

% --------------------
\subsection{Signal Abuse}
%
\label{sec:secevalscall}
% --------------------

% --------------------
\subsection{Probabilistic Analysis of Leakage}
%
\label{sec:secevalrand}
% --------------------


==> space_tricks.tex <==
% %space left between floats.
\setlength{\floatsep}{1mm}
% % space between last top float or first bottom float and the text.
\setlength{\textfloatsep}{2mm}
% % space left on top and bottom of an in-text float.
\setlength{\intextsep}{2mm}
% % space above caption
\setlength{\abovecaptionskip}{1mm}
% %space below caption
\setlength{\belowcaptionskip}{2mm}
% %like textfloatstep for 2 column figures
\setlength{\dbltextfloatsep}{2mm}
% %like floatstep for 2 column figures
\setlength{\dblfloatsep}{2mm}
%
% %% Change figure handling
% \renewcommand{\topfraction}{0.999999}
% \renewcommand{\textfraction}{0.00001}
% \renewcommand{\floatpagefraction}{0.9999999}

%\usepackage{bibspacing}
%\setlength{\bibspacing}{24pt}

% \usepackage{tweaklist}
% \renewcommand{\enumhook}{\setlength{\topsep}{0pt}
%   \setlength{\itemsep}{0pt}}
% \renewcommand{\itemhook}{\setlength{\topsep}{0pt}
%   \setlength{\itemsep}{0pt}}
%% \renewcommand{\descripthook}{\setlength{\topsep}{0pt}
%   \setlength{\itemsep}{0pt}}

%\usepackage[compact]{titlesec}
%
%\usepackage{titling}
%\setlength{\droptitle}{-3em}
%
 %\setlength{\parskip}{0pt}
 %\setlength{\parsep}{0pt}
 %\setlength{\headsep}{0pt}
 %\setlength{\topskip}{0pt}
 %\setlength{\topmargin}{0pt}
 %\setlength{\topsep}{0pt}
 %\setlength{\partopsep}{0pt}


==> specification.tex <==
\newcommand{\SP}[1]{\mathbf{SP}_{#1}}
\newcommand{\ST}{\mathbf{S}}
\newcommand{\State}[1]{\mathbf{#1}}
\newcommand{\T}{\mathbf{T}}
\newcommand{\U}{\mathbf{U}}
\newcommand{\tran}{\tau}
\newcommand{\pre}{\mathtt{pre}}

\newcommand{\fct}[1]{\mathtt{#1}}

%%----------------------------------------------------------
\section{Specifying a secure OS Interface for intra-process Isolation}
%%----------------------------------------------------------

    % --------------------
    Goal of this section is to define the specification of OS interface in the
    presence of intra-process compartments which protects each compartment's
    confidentiality and integrity of memory.
    %%
    We focus on the OS interface of Linux for this purpose which consists of XXX
    system calls and pseudo files such as files located in /proc.
    %%
    What high level properties do we want to protect?
    %%
    Trusted monitor conf. + integrity from untrusted application
    % -------------------

    % -------------------
    Paragraph about why sys calls may violate these properties
    % -------------------

    % -------------------
    Non goals of this specification/assumptions are:
    %%
    1. not trying to specify the safety of the system call interception technique
    %%
    2. not trying to specify the safety of the memory isolation technique itself
    % -------------------

\subsection{Defining a Framework for intra-process Memory Isolation}

    % -------------------
    Implement a state machine with transition functions $\tran$ between states
    $\ST$.
    %%
    A state $\ST$ from $\State{Q}$ describes the current memory mappings and
    thier protection.
    %%
    Transition functions are interactions with the OS like system calls or
    accesses to pseudo files of the OS. State $\ST$ may only transition $\ST'$
    via $\tran_i$, if the precondition $\pre(\ST)$ evaluates successfully.
    % -------------------

    % -------------------
    \paragraph{State $\ST$} represents all memory, its permissions, and what it
    is mapped to on the file system and is a tuple of
    \[ \ST = (\State{M} \times \State{MP} \times \State{MF} \times \State{OF}
    \times \State{FS} \times \State{D}) \]
    %%
    $\State{M}$ represents the set of mapped memory addresses.
    %%
    \[
        \State{M} = \{ addr | addr : \mathbb{N} \}
        \]
    %%
    $\State{MP}$ represents the function from an address to its memory domain
    and permission.
    %%
    \[
        \State{MP}: addr : \mathbb{N} \rightarrow (d : \State{D} \times perm :
        (R, W, X))
        \]
    %%
    $\State{MF}$ represents the set of addresses $addr$ which are mapped to the
    interval $[off, len]$ of a file descriptor.
    %%
    \begin{equation}
        \begin{aligned}
            \State{MF} = & \{(fd, off, len, addr) |  \\
            & \exists addr \in \State{M}:  \fct{map}(fd, off, len) = addr\}
        \end{aligned}
    \end{equation}
    %%
    $\State{OF}$ represents the set of open files. (not sure if we really need
    it)
    %%
    \[
        \State{OF} = \{fd : \mathbb{N} | \exists p \in \State{FS}: \fct{open}(p)
         = fd\}
    \]
    %%
    $\State{FS}$ represents the file system state as a function of path to file
    descriptor.
    %%
    \[
        \State{FS} = \{path : string | \fct{exists}(path)\}
    \]
    %%
    $\State{D}$ represents the currently running domain either $\T$ for trusted
    or one of the untrusted domains $\U_i$.
    %%
    \[
        \State{D} \rightarrow d : \{\T, \U_0, ..., \U_n\}
    \]
    % -------------------

    % -------------------
    Initial state that every program starts with has the loader and security
    monitor in trusted memory and no files have been opened or mapped. The
    current domain is trusted.
    % -------------------

    % -------------------
    Safety properties are the once we try to achieve.
    % -------------------

    \noindent $\SP{1}$: When execution is untrusted, trusted memory cannot be
    read.

    \noindent $\SP{2}$: When execution is untrusted, trusted memory cannot be
    written.

    \noindent $\SP{3}$: Disallow memory permission of writeable and
    executable.

    \noindent $\SP{4}$: Disallow aliasing of memory

    \[
        \forall a \in \State{M}: \State{P}(a) = (\T, \_) \land \State{D} = \U
        \rightarrow \neg \fct{readable}(a)
        \tag{$\SP{1}$} \label{spec:sp1}
    \]\[
        \forall a \in \State{M}: \State{P}(a) = (\T, \_) \land \State{D} = \U
        \rightarrow \neg \fct{writeable}(a)
        \tag{$\SP{2}$} \label{spec:sp2} \\
    \]\[
        \forall a \in \State{M}: \fct{writeable}(a) \oplus \fct{executable}(a)
        \tag{$\SP{3}$} \label{spec:sp3}
    \]\begin{equation}
        \begin{aligned}
        \forall mf \in \State{MF}: & \nexists mf' \in \State{MF}: \\
         & \State{P}(mf.addr).domain \neq \State{P}(mf'.addr).domain \\
        \land & mf.fd = mf'.fd \\
        \land & \fct{offset\_intersects}(mf, mf')
        \end{aligned}
        \tag{$\SP{4}$} \label{spec:sp4}
    \end{equation}
    % -------------------

    % -------------------
    A state is called safe, if all safety properties are met. We build a safety
    framework by transition safety and sequential composition safety.
    %%
    \[
        \ST \models \SP{1} \land \SP{2} \land \SP{3} \land \SP{4} \rightarrow
        \fct{safe}(\ST)
        \tag{Safety} \label{spec:safety}
    \]
    % -------------------

    % -------------------
    \paragraph{Transition safety:} A safe state $\ST$ transitioning via
    $\tran_i$ to state $\ST'$, satisfying the preconditions $\pre_i$ of
    $\tran_i$, leads to a safe sate $\ST'$.
    %%
    \[
        \forall \ST, \ST' \in \State{Q}, i: \fct{safe}(S) \land \pre_i(\ST)
        \rightarrow \tran_i(\ST,\ST') \land \fct{safe}(\ST')
        \label{spec:transafety}
    \]
    % -------------------

    % -------------------
    \paragraph{Sequential composition safety:} From transition safety we can
    observe that a chain of states $\ST_1 \ldots \ST_n$ connected via
    transitions $\tran_1 \ldots \tran_{n-1}$ leads to a safe state $\ST_n$ by
    enforcing transition safety on every step.
    %%
    \begin{equation}
        \begin{aligned}
        \ST_0, \ldots, \ST_n \in \State{Q}: & \tran_0, \ldots, \tran_{n-1}: \\
        \fct{safe}(\ST_0) \rightarrow &
         \tran_0(\ST_0, \ST_1) \land \ldots \land
        \tran_{n-1}(\ST_{n-1}, \ST_n) \\
        \land & \fct{safe}(\ST_n)
        \end{aligned}
    \end{equation}
    % -------------------

    % -------------------
    This allows us to do a prove by induction from a well defined initial state
    or contradiction (which might be easier for the paper - kind of if there was
    such a violation).
    % -------------------

    % -------------------
    \paragraph{Transition functions $\tran$} represent the interactions
    between states.
    %%
    In this particular instance, we identified system calls which may alter the
    respective memory permissions, mappings, or directly access memory
    information.%%
    Table XXX shows the pre-condition for each system call and the state
    transition.
    %%
    In addition, we also describe a general transition between trusted and
    untrusted via $switch$.
    %%
    This construction is necessary, since the trusted monitor may do system
    calls independent of the untrusted execution.
    % -------------------





==> tramps.tex <==
% --------------------
\subsubsection{\syscall Instruction Capabilities}
% --------------------

% --------------------
We consider \syscall as a privilege in \system. Which means any attempts of 
invoking \syscall must execute the \syscall with a deterministic control flow 
starts from any \syscall entrypoints. This ensures the proper sanity checks are 
performanced for the syscalls. 
To do so, we propose \emph{\stramp}.
It consists a method to restrict the \syscall within the \system that guaranteed the control flow integrity,
and a method to enforce control flow integrity at least in \system.
%
We could use the same approach to protect \wrpkru, however, the bytecode
sequence for \syscall is much smaller and more likely to occur in the benign \ud
code.
%
The first property is straightforward, \ie no direct access to \syscall
instructions. It can be provided by seccomp---which has the powerful side effect of
eliminating the seccomp attack presented in PKU Pitfalls~\cite{Connor:PKU:2020}. 

However, the seccomp filter has its own limitation, once the policies are loaded, 
they can no longer be retreated nor disabled. 
This is okay when only one thread is needed, however it might be problemastic 
in certain configuraion with multithreading if the control flow integrity is not 
CET based. Because all threads are sharing the same memory space and as a result, 
the share the same address for legal \syscall that cannot be modified. Causing 
performance issue when multiple threads must synchronize for the only \syscall, 
and also security issue since a exploitable syscall gadget will be exposed to all threads
when some of them might in the \ud. 

Also, during the evaluation we found that by enabling the seccomp filter will introduce
much overhead.

Syscall User Dispatch~\cite{dispatch} is a recent kernel patch that destined for
Linux 5.11. Compared to seccomp, it provides a simply but power interface to restrict 
a given IP range that is allowed for invoking \syscall. Any \syscall outside this range 
will fail automatically. 


